Topologically simple infinite matrix groups indexed by ordered sets

This article focuses on the study of the group of units of incidence rings, which is a class of infinite matrix groups indexed by ordered sets, on a topological perspective. We first show when these groups can inherit the topological structure from the incidence rings. It is later shown that infinite matrix groups of topological fields can be used to build simple topological matrix groups, generalizing a result proven in ``Topologically simple, totally disconnected, locally compact infinite matrix groups''. We finish by relating the structure of these groups with elementary totally disconnected, locally compact groups, an important class for the study of totally disconnected, locally compact groups.

==> Sections/3-Rings.tex <==
\section{Topological incidence rings}\label{rings_construction}

\subsection{First definitions}

\begin{defi}\cite[Definition 1.1]{Matrices1973}\label{defi:proset matrices}\index{$\textup{M}_{\Lambda}(P)$|ndx}\index{ring of matrices indexed by a proset|ndx}
Let $P$ be a ring and $(\Lambda,\  \preceq)$ a locally finite proset. We define the \textbf{incidence ring of $\Lambda$ over $P$} as
$$\textup{M}_\Lambda(P):=\left\{ (a_{s_1,s_2})\in P^{\Lambda\times \Lambda}
: \textit{ if }a_{s_1,s_2}\neq 0\textit{ then } s_1  \preceq s_2 \right\}$$
with  coordinatewise sum and multiplication defined as follows: given two element $(a_{s_1,s_2}),(b_{s_1,s_2})\in \textup{M}_\Lambda(P)$ then $(a_{s_1,s_2}).(b_{s_1,s_2})=(c_{s_1,s_2})$,\ where $c_{s_1,s_2}=\sum_{t\in[s_1,s_2]}a_{s_1,t}b_{t,s_2}$. 
\end{defi}

Note that this multiplication is defined in such a way that for any finite $n\times n$ block of the matrix centered on the main diagonal,\ the multiplication follows the same rule as $\textup{M}_\mathbf{n}(P)$. We will denote the elements of $\textup{M}_\Lambda(P)$ as $A,B,C$. We denote $A_{s_1,s_2}$ as the coordinate $(s_1,\ s_2)$ in the matrix $A$. When talking about the coordinate of the product $A_1A_2\ldots A_n$ we denote it as $(A_1A_2\ldots A_n)_{s_1,s_2}$. Following are some examples of incidence rings.

\begin{ex}
\begin{enumerate}
    \item Given $n\in\mathbb{N}$,\ the ring $\textup{M}_{\mathbf{n}}(P)$ is the ring of $n\times n$ matrices over the ring $P$ with the usual multiplication.
    \item Given $n\in\mathbb{N}$,\ the ring $\textup{M}_{\mathbf{n<}}(P)$ is the ring of $n\times n$ upper triangular matrices over $P$ with the usual multiplication.
    \item Given $S$ a set,\ the ring $\textup{M}_S(P)$ is isomorphic to $\prod_{s\in S} P$ with the coordinate-wise multiplication. 
    \item The ring $\textup{M}_{\mathbf{N}^*_d}(P)$ has elements of the form:

$$
A:=\left(\begin{array}{cccccc}
A_{1,1} & A_{1,2} & A_{1,3} & A_{1,4} & A_{1,5}  & \cdots \\
0 & A_{2,2} & 0 & A_{2,4} & 0 & \cdots\\
0 & 0 & A_{3,3} & 0 & 0  & \cdots \\
0 & 0 & 0 & A_{4,4} & 0 &  \cdots \\
0 & 0 & 0 & 0 & A_{5,5} &  \cdots  \\
0 & 0 & 0 & 0 & 0 &  \cdots \\
\vdots & \vdots  & \vdots & \vdots & \vdots & \ddots
\end{array}\right)
$$

\noindent and the multiplication of two matrices $A,B\in \textup{M}_{\mathbf{N}^*_d}(P)$ is:

$$
A
B:=\left(\begin{array}{ccccccc}
A_{1,1}B_{1,1} & \sum_{d|2}A_{1,d}B_{d,2} & \sum_{d|3}A_{1,d}B_{d,3} & \sum_{d|4}A_{1,d}B_{d,4} & \sum_{d|5}A_{1,d}B_{d,5}  & \cdots \\
0 & A_{2,2}B_{2,2} & 0 & \sum_{d|4}A_{2,d}B_{d,4} & 0 & \cdots\\
0 & 0 & A_{3,3}B_{3,3} & 0 & 0 &  \cdots \\
0 & 0 & 0 & A_{4,4}B_{4,4} & 0 &  \cdots \\
0 & 0 & 0 & 0 & A_{5,5}B_{5,5} &  \cdots  \\
0 & 0 & 0 & 0 & 0 &  \cdots \\
\vdots & \vdots  & \vdots & \vdots & \vdots & \ddots
\end{array}\right)
$$
\end{enumerate}
\end{ex}
Given $S\subset \textup{M}_{\Lambda}(P)$ a subset,\ we define $S_{s_1,s_2}=\{A_{s_1,s_2}:\ A\in S\}\subset P$. Note though that $R\subset \textup{M}_\Lambda(P)$ a subset is a subring if $0,1\in R$ and for every $s_1  \preceq s_2$ in $\Lambda$ we have that
$$R_{(s_1,s_2)}+R_{(s_1,s_2)}\subset R_{(s_1,s_2)},$$
$$\sum_{s\in[s_1,s_2]}R_{s_1,s}R_{s,s_2}\subset R_{s_1,s_2}.$$
And $I\subset \textup{M}_{\Lambda}(P)$ a subset is a two-sided ideal if $0\in I$ and for every $s_1  \preceq s_2$ in $\Lambda$ we have that
$$R_{(s_1,s_2)}+R_{(s_1,s_2)}\subset R_{(s_1,s_2)},$$
$$\sum_{s\in[s_1,s_2]}I_{s_1,s}R_{s,s_2}\subset I_{s_1,s_2},$$
$$\sum_{s\in[s_1,s_2]}R_{s_1,s}I_{s,s_2}\subset I_{s_1,s_2}.$$
This allows us to easily describe some ideals and subrings of $\textup{M}_{\Lambda}(P)$ central to our work. These also allow us to prove the existence of a topology on $\textup{M}_\Lambda(P)$ in a natural way,\ preserving properties of the finite blocks of matrices.

\begin{notation}[Ideals of $\textup{M}_\Lambda(P)$]\label{defi:ideals}
Let $\Lambda$ a locally finite proset and $P$ a ring. We denote the following two-sided ideals:
\begin{itemize}
    \item Given $s_1  \preceq s_2$ in $\Lambda$ we define 
    $$I^{\Lambda}_{[s_1, s_2]}(P)=\{A\in \textup{M}_{\Lambda}(P):\ \text{ if } t_1,\ t_2\in[s_1,\ s_2] \text{ then } A_{t_1,t_2}=0 \}.$$ 
    This ideal has quotient 
    $$\textup{M}_{\Lambda}(P)/I^{\Lambda}_{[s_1,s_2]}(P)\cong \textup{M}_{[s_1,s_2]}(P).$$
    \item For a convex set $\Lambda'\subset \Lambda$,\ the ideal
    $$I^{\Lambda}_{\Lambda'}=\bigcap_{s_1  \preceq s_2\in \Lambda'}I^{\Lambda}_{[s_1,s_2]}.$$
    This ideal has quotient $$\textup{M}_{\Lambda}(P)/I^{(\Lambda,\  \preceq)}_{\Lambda'}\cong \textup{M}_{\Lambda'}(P).$$
    \item For $\{\Lambda_i\}_{i\in I}$ a locally convex set of $\Lambda$ we define the ideal 
    $$I^{\Lambda}_{\{\Lambda_i\}_{i\in I}}=\bigcap_{i\in I}I^{\Lambda}_{\Lambda_i}.$$
    This ideal has quotient 
    $$\textup{M}_{\Lambda}(P)/I^{\Lambda}_{\{\Lambda_i\}_{i\in I}}\cong \prod_{i\in I} \textup{M}_{\Lambda_i}(P).$$
    \item Given $J\leqslant P$ a two-sided ideal we define
    $$\textup{M}_{\Lambda}(J):=\{A\in \textup{M}_\Lambda(P): \text{ for every } t_1,t_2\in \Lambda \text{ then } A_{t_1,t_2}\in J \}\leqslant \textup{M}_\Lambda(P).$$
    This ideal has quotient 
    $$\textup{M}_\Lambda(P)/\textup{M}_\Lambda(J)\cong \textup{M}_\Lambda(P/J).$$
    \item  Given $\{\Lambda_i\}_{i\in I}$ a locally convex set of $\Lambda$ and $J\leqslant P$ a two-sided ideal of $P$,\ then the ideal $$I_{\{\Lambda_i\}_{i\in I}}+\textup{M}_\Lambda(J)$$
    has quotient 
    $$\textup{M}_\Lambda(P)/(I_{\{\Lambda_i\}_{i\in I}}+\textup{M}_\Lambda(J))\cong \prod_{i\in I} \textup{M}_{\Lambda_i}(P/J).$$
\end{itemize} 
\end{notation}

Some of the ideals above were initially defined at \cite{Matrices1973}.

\begin{ex}
In the case of the matrix ring $\textup{M}_\mathbf{N}(\mathbb{Z}_p)$ and interval be $[0,\ 2]=\{0,\ 1,\ 2\}$,\ we have that $I_{[0,2]}$ has elements of the form
$$
\left(\begin{array}{cccccc}
0 & 0 & 0 & A_{0,3} & A_{0,4}  & \cdots \\
0 & 0 & 0 & A_{1,3} & A_{1,4} & \cdots\\
0 & 0 & 0 & A_{2,3} & A_{2,4}  & \cdots \\
0 & 0 & 0 & A_{3,3} & A_{3,4} &  \cdots \\
0 & 0 & 0 & 0 & A_{4,4} &  \cdots  \\
\vdots & \vdots  & \vdots & \vdots & \vdots & \ddots
\end{array}\right)
$$
and the quotient $\textup{M}_\mathbf{N}(\mathbb{Z}_p)/I_{[0,2]}$ is isomorphic to $\textup{M}_{\mathbf{3<}}(\mathbb{Z}_p)$,\ the ring of upper $3\times 3$ triangular matrices over $\mathbb{Z}_p$. Given the ideal $p\mathbb{Z}_p$ of $\mathbb{Z}_p$,\ the quotient $\textup{M}_\mathbf{N}(\mathbb{Z}_p)/\textup{M}_\mathbf{N}(p\mathbb{Z}_p)$ is isomorphic to $\textup{M}_\mathbf{N}(\mathbb{Z}/p\mathbb{Z})$,\ and  $\textup{M}_\mathbf{N}(\mathbb{Z}_p)/(I_{[0,2]}+\textup{M}_\mathbf{N}(p\mathbb{Z}_p))$ is isomorphic to $\textup{M}_{\mathbf{3<}}(\mathbb{Z}/p\mathbb{Z}).$
\end{ex}




\subsection{Infinite matrices as limits of finite matrices}

To prove the results in this section we will look at $\textup{M}_\Lambda(P)$ as objects in the category of associative topological rings with identity and the morphisms are the continuous homomorphism of rings. This category will be denoted as $\textbf{TopRings}$. For the next result,\ notice that if $P$ is a topological ring and $\Lambda$ is a finite proset,\ then the ring $\textup{M}_\Lambda(P)$ is a topological ring with subspace topology in relation to the product space $P^{\Lambda\times\Lambda}$. In a similar way, for $\Lambda$ an infinite, locally finite proset we define the topology on $\textup{M}_{\Lambda}(P)$ as the subspace topology on $P^{\Lambda\times \Lambda}$. Our main goal in this subsection is proving that with this topology, $\textup{M}_{\Lambda}(P)$ is a topological ring.\\
\indent Notice that if $\Lambda'\subset \Lambda$ is a finite convex subset,\ say $\Lambda'=\{s_1,\ s_2,\ \ldots,\ s_n\}$,\ then $\textup{M}_{\Lambda'}(P)$ can be seen as a subring of $\textup{M}_{\mathbf{n}}(P)$ with embedding determined by the enumeration of $\Lambda'$. The ideals of the form $I^\Lambda_{\Lambda'}$,\ for $\Lambda'$ a finite convex subset,\ will then be essential to build our inverse limit and the topology,\ as the quotient under such ideals are topological incidence rings.\\
\indent Given $\Lambda$ a proset,\ define $\Gamma(\Lambda)=\{\alpha\subset \Lambda:\  \alpha\text{ is finite and convex}\}$ \textbf{the set of all finite convex subsets of $\Lambda$}. The next result follows directly from Proposition \ref{prop:finite subsets into finite convex}.\index{$\Gamma(\Lambda)$|ndx}\index{set of finite, convex subsets of a proset|ndx}

\begin{coro}\label{coro:directed set}
If $\Lambda$ is an irreducible poset then for convex subsets $\alpha,\ \beta\in \Gamma(\Lambda)$ there is $\gamma\in \Gamma(\Lambda)$ such that $\alpha\subset \gamma$ and $\beta\subset \gamma$,\ that is,\ under the $\subset$ order the set $\Gamma(\Lambda)$ is a directed set.
\end{coro}
%\begin{proof}
%By Proposition \ref{prop:finite subsets into finite convex} it follows that,\ because $\alpha,\ \beta$ are finite there exists $\gamma$ such that $\gamma$ is convex and $\alpha,\beta\subset \gamma$.
%\end{proof}

%Notice that this definition implies that the quotient of such matrix rings under $I_{\Lambda'}$ (Notation \ref{defi:dense subset}) is continuous. Some examples of rings satisfying these properties are any discrete rings,\ locally compact topological fields and prodiscrete rings.

We can then prove the following Theorem:
\begin{theorem}\label{Prop: prodiscrete ring}
Let $P$ a ring and $(\Lambda,\  \preceq)$ an infinite irreducible locally proset. Then $\textup{M}_\Lambda(P)\cong\varprojlim_{\alpha\in\Gamma(\Lambda)} \textup{M}_\alpha(P)$. If $P$ is a topological ring then $\textup{M}_{\Lambda}(P)$ is a topological ring with topology given by the inverse limit.
\end{theorem}

\begin{proof}

By Corollary \ref{coro:directed set} we have that $\Gamma(\Lambda)$ is a directed set. Given $\alpha\subset \beta\in \Gamma(\Lambda)$ define $\pi_{\beta\rightarrow\alpha}:\textup{M}_\beta(P)\longrightarrow \textup{M}_\alpha(P)$ as the natural projection of $\textup{M}_\beta(P)$ with kernel $I^{\beta}_{\alpha}$. It is easy to see that given $\alpha\subset\beta\subset\gamma$ then $\pi_{\gamma\rightarrow\alpha}=\pi_{\beta\rightarrow\alpha}\circ \pi_{\gamma\rightarrow\beta}$,\ that is,\ the following diagram commutes.\\
\begin{center}
\begin{tikzcd}
% https://tikzcd.yichuanshen.de/#N4Igdg9gJgpgziAXAbVABwnAlgFyxMJZARgBoAGAXVJADcBDAGwFcYkQAVAJywAoAdfgHN6AW1H0AlCAC+pdJlz5CKcqWLU6TVu259BAIxg4ps+SAzY8BIgCZ1mhizaJOPAfyZoAFqZmaYKCF4IlAAMy4IUSQ1EBwIJHstZ3ZBNCwAfWBBEXF6QR4hbxMuSIB3QS9fGRAaRnojRgAFRWsVECwwbFgzcMjoxFj4pDJknVc0zOzhMQkCrCKS8sNjehq6hphm1uV2Tu62OT6okZphxCSncZBJrJWTecX6UogKz0YfNdqQesaWq12rn2WB6-hkQA
                                                                  & \textup{M}_\gamma(P) \arrow[rd, "\pi_{\gamma\rightarrow\alpha}" description] \arrow[ld, "\pi_{\gamma\rightarrow\beta}" description] &             \\
\textup{M}_\beta(P) \arrow[rr, "\pi_{\beta\rightarrow\alpha}" description] &                                                                                                                            & \textup{M}_\alpha(P)
\end{tikzcd}
\end{center}

The collection $((\textup{M}_{\alpha})_{\alpha\in \Gamma(\Lambda)},(\pi_{\beta\rightarrow\alpha})_{\alpha\subset\beta})$ is then an inverse system. As the category of associative rings with identity is closed under inverse limits,\ the inverse limit of this system exists and is unique. Denote $\varprojlim_{\alpha\in\Gamma(\Lambda)} \textup{M}_\alpha(P)$ as the inverse limit of this system. Our objective now is proving $\textup{M}_\Lambda\cong \varprojlim_{\alpha\in\Gamma(\Lambda)} \textup{M}_\alpha(P)$.\\
\indent Observe that for every $\alpha\in\Gamma(\Lambda)$ there is $\psi_{\alpha}:\textup{M}_\Lambda(P)\longrightarrow \textup{M}_\alpha(P)$ given by the natural projection of $\textup{M}_\Lambda$ under $I^\Lambda_{\alpha}$,\ and these projections are such that the outer triangle of the following diagram commutes.
\\

\begin{center}
% https://tikzcd.yichuanshen.de/#N4Igdg9gJgpgziAXAbVABwnAlgFyxMJZAJgBoAGAXVJADcBDAGwFcYkQAVAJywAoAdfgBl6AWwBGUegEoQAX1LpMufIRRkAjNTpNW7APTzFIDNjwEiZYtoYs2iEIIZc0XCACtGWUQH1ggpjQAC3pBLDBBAHExUXoBYTFJGTkAAm4+AMZgmSMlM1UiclIAZhtde04eeMCQn2JZBTyVCxQAFhKyu3Z06qzajQbtGCgAc3giUAAzN1EkIpAcCCQyHS6HSZAaRnpxGEYABWVzNRBw7FhNkC8wCqk4IOHckGmIWcR5xaR21b0HQTRsH5MtkfBo5JdtrsDkcCg4zlgLo1njM5jRPohijRbL9HPwAVggfwavQ6uCtjs9od8i1TmBzmwkS83it0d9sRV-gT-ES+iSwRCKdDqSd4YjjEzlmilhiseV2JzCcTSQKoVTmiK6QiGeKUTKFtK2XK-niucDasRBDwRkEcPQuG4AO5mvlkq6CtXHdiihmUORAA
\begin{tikzcd}
                                                                            &  & \textup{M}_\Lambda(P) \arrow[dd, "f" description, dashed] \arrow[rrddd, "\psi_{\alpha_1}" description] \arrow[llddd, "\psi_{\alpha_2}" description] &  &               \\
                                                                            &  & /                                                                                                                                          &  &               \\
                                                                            &  & \varprojlim_{\alpha\in\Gamma(\Lambda)} \textup{M}_\alpha(P) \arrow[rrd, "\pi_{\alpha_1}" description] \arrow[lld, "\pi_{\alpha_2}" description]     &  &               \\
\textup{M}_{\alpha_2}(P) \arrow[rrrr, "\pi_{\alpha_2\rightarrow\alpha_1}" description] &  &                                                                                                                                            &  & \textup{M}_{\alpha_1}(P)
\end{tikzcd}
\end{center}


By the universal property of inverse limits,\ there exists an unique ring homomorphism $f:\textup{M}_\Lambda(P)\longrightarrow \varprojlim_{\alpha\in\Gamma(\Lambda)} \textup{M}_\alpha(P)$ such that the whole diagram commutes. It remains to show the function $f$ is a bijection.\\
\indent Let $A\in \textup{M}_\Lambda(P)$ be such that $f(A)=0$. Because the diagram commutes we have that $\psi_{\alpha}(A)=0$ for all $\alpha\in\Gamma(\Lambda)$. Because these projections are such that $\psi_{\alpha}(A)=0$ if,\ and only if,\ $A_{t_1,t_2}=0$ for all $t_1,\ t_2\in\alpha$ we have that $A=0$. Hence $f$ is injective.\\
\indent It remains to prove that $f$ is surjective. For that,\ given $\overline{A}\in \varprojlim_{\alpha\in\Gamma(\Lambda)} \textup{M}_\alpha(P)$ we need to find $A\in \textup{M}_\Lambda(P)$ such that $f(A)=\overline{A}$. We will describe such $A$ coordinate-wise. Notice that as $f$ is a ring homomorphism,\ it will an isomorphism if,\ and only if,\ $f$ is an isomorphism of abelian groups (when we forget the multiplication structure on our ring). Hence we can treat these as abelian groups to simplify our proof.\\
\indent Observe that by looking at these as abelian groups,\ for every proset $\Lambda$ we have that $\textup{M}_\Lambda(P)$ is a subgroup of $P^{\Lambda\times \Lambda}$. Hence for every $s_0,\ t_0\in \Lambda$ there is a projection $$\begin{array}{c}
\pi^\Lambda_{s_0,t_0}:\textup{M}_\Lambda(P)\rightarrow P\\
A\mapsto A_{s_0,t_0}.
\end{array}$$ 
Similarly,\ for $\alpha_1,\alpha_2\in\Gamma( \Lambda)$,\ with $\alpha_1\subset\alpha_2$,\ and $s_0,\ t_0\in\alpha_1$ there are projection $\pi^{\alpha_1}_{s_0,t_0}:\textup{M}_{\alpha_1}(P)\rightarrow P$ and $\pi^{\alpha_2}_{s_0,t_0}:\textup{M}_{\alpha_2}(P)\rightarrow P$ such that $\pi_{s_0,t_0}^{\alpha_1}\circ \psi_{\alpha_1}=\pi_{s_0,t_0}^{\alpha_2}\circ \psi_{\alpha_2}$,\ and the  following diagram commutes:
\begin{center}
% https://tikzcd.yichuanshen.de/#N4Igdg9gJgpgziAXAbVABwnAlgFyxMJZAJgBoAGAXVJADcBDAGwFcYkQAVAJywAoAdfgBl6AWwBGUegEoQAX1LpMufIRRkAjNTpNW7APTzFIDNjwEiZYtoYs2iEIIZc0XCACtGWUQH1ggpjQAC3pBLDBBAHExUXoBYTFJGTkAAm4+AMZgmSMlM1UiclIAZhtde04eeMCQn2JZBTyVCxQAFhKyu3Z06qzajQbjU2a1ElJWzr0HAAV5bRgoAHN4IlAAMzdRJCKQHAgkMh0uhzWQGkZ6cRhGaeVzNRBw7FgzkC8wCqk4IIXckA2IFtEDs9kh2kcpo5+GhsH5MtkfBo5K8LlcbncCg4nlgXo1-pttjRQYhijRbJDBDCsHD+DV6HVkedLtdbvkWo8wM82HiAUDDsTweSKpTqf5aX16UiUcz0WyHtjccZeQcifsSWTyuwRTS6QzpWjWSN2AruUqCerdmrBZqHNqxbriIIeIsgjh6Fw3AB3eH9RlvGWG+7Gzk403rc2ky1IACsTINGPZJteQq10KwAD17RKGX44D4ijh88ieebwcTY-743Lg1zkzaoWgM1mEUjc-nSIXyMXKHIgA
\begin{tikzcd}
                                                                                                                                  &  & \textup{M}_\Lambda(P) \arrow[dd, "f" description, dashed] \arrow[rrddd, "\psi_{\alpha_1}" description] \arrow[llddd, "\psi_{\alpha_2}" description] &  &                                                                    \\
                                                                                                                                  &  & /                                                                                                                                          &  &                                                                     \\
                                                                                                                                  &  & \varprojlim_{\alpha\in\Gamma(\Lambda)} \textup{M}_\alpha(P) \arrow[rrd, "\pi_{\alpha_1}" description] \arrow[lld, "\pi_{\alpha_2}" description]     &  &                                                                     \\
\textup{M}_{\alpha_2}(P) \arrow[rrrr, "\pi_{\alpha_2\rightarrow\alpha_1}" description] \arrow[rrd, "{\pi^{\alpha_2}_{s_0,t_0}}" description] &  &                                                                                                                                            &  & \textup{M}_{\alpha_1}(P) \arrow[lld, "{\pi^{\alpha_1}_{s_0,t_0}}" description] \\
                                                                                                                                  &  & P                                                                                                                                          &  &                                                                    
\end{tikzcd}
 \end{center}

\noindent That is,\ the coordinate $A_{s_0,t_0}$ is the same for all $\alpha\in\Gamma(\Lambda)$ such that $s_0,\ t_0\in\alpha$.\\
\indent Notice that $\pi_{s_0,t_0}^{\beta_1}\circ\pi_\alpha(\overline{A})=\pi_{s_0,t_0}^{\beta_2}\circ\pi_\alpha(\overline{A})$ for every $\beta_1,\ \beta_2\in \Gamma(\Lambda)$ such that $[s_0,\ t_0]\subset \beta_i$,\ $i=1,\ 2$. We define $A$ coordinatewise as $A_{s_0,t_0}=\pi^{\alpha}_{s_0,t_0}\circ\pi_{\alpha}(\overline{A})$,\ for $s_0,\ t_0\in \alpha$ and $\alpha\in\Gamma(\Lambda)$. As the diagram commutes,\ $\pi^\alpha_{s_0,t_0} \circ \pi_{\alpha} \circ f=\pi^\alpha_{s_0,t_0}\circ\psi_{\alpha}$ for all $s_0  \preceq t_0$ such that $s_0,\ t_0\in \alpha$, and $\alpha\in\Gamma(\Lambda)$. Hence $A$ is so that $f(A)=\overline{A}$. That is,\ $f$ is an isomorphism of rings.\\
\indent By the inverse limit property,\ $\textup{M}_\Lambda(P)$ is a closed subset of $\prod_{\alpha\in \Gamma(\Lambda)}\textup{M}_{\alpha}(P)$ under the product topology,\ hence it can be seen as a topological ring.\\
\indent Notice that,\ as observed earlier for finite prosets,\ it then follows that $\textup{M}_\Lambda(P)$ is a closed subset of $\prod_{\alpha\in\Gamma(\Lambda)}P^{\alpha\times \alpha}$. As $\Lambda$ is infinite,\ we have that $|\Gamma(\Lambda)|=|\Lambda|$. Hence there exists a homeomorphism between $\prod_{\alpha\in\Gamma(\Lambda)}P^{\alpha\times \alpha}$ and $P^{\Lambda\times \Lambda}$ given by a bijection from $\bigsqcup_{\alpha\in \Gamma{(\Lambda)}}\alpha\!\times\! \alpha$ to $\Lambda\!\times\!\Lambda$. That is,\ the topological ring structure on $\textup{M}_\Lambda(P)$ can be seen as the subspace topology in relation to $P^{\Lambda\times \Lambda}$,\ as in the finite proset case.
\end{proof}


\begin{prop}\cite[Lemma 2.2]{Matrices1985}\label{prop:disjoint union and product rings}
Let $P$ be a ring and $\Lambda=\sqcup_{i\in I}\Lambda_i$ a preordered set. Then $\textup{M}_{\Lambda}(P)\cong \prod_{i\in I}\textup{M}_{\Lambda_i}(P)$. If $P$ is a topological ring then $\textup{M}_{\Lambda}(P)$ is a topological ring with topology given by the product topology on the $\textup{M}_{\Lambda_i}(P)$.
\end{prop}

%\begin{proof}
%Let $A\in \textup{M}_{\Lambda}(P)$. Define,\ for each $i\in I$ the surjective homomorphisms $\pi_i:\textup{M}_{\Lambda}(P)\rightarrow \textup{M}_{\Lambda_i}(P)$ coordinatewise as $\pi_i(A)_{s_1,s_2}:=  A_{s_1,s_2}$ if $s_1,\ s_2\in \Lambda_i$. Given $R$ a ring and,\ for every $i\in I$,\ a map $f_i:R\rightarrow \textup{M}_{\Lambda_i}(P)$ one can define $f:R\rightarrow \textup{M}_\Lambda(P)$ coordinatewise as:
%$$f(r)_{s_1,s_2}:=\left\{\begin{array}{ll}
%   f_i(r)_{s_1,s_2}  & \mbox{if }s_1,\ s_2\in \Lambda_i  \\
 %   0 & \mbox{otherwise.}
%\end{array}\right.$$
%\noindent This is clearly a ring homomorphism and satisfy $f_i=\pi_i\circ f$ for every $i\in I$. Hence the result follows.
%\end{proof}
Notice that Theorem \ref{Prop: prodiscrete ring} and Proposition \ref{prop:disjoint union and product rings} implies that all matrix rings indexed by prosets are limits of finite matrix rings. Both results then imply that the topology given to $\textup{M}_{\Lambda}(P)$ in relation to $\textup{P}^{\Lambda\times \Lambda}$ makes $\textup{M}_{\Lambda}(P)$ into a topological ring. More than that, this is the topology given by the inverse limit.\\
\indent For an example,\ let $\mathbf{2}\!<$ be our poset and $P$ be any ring. We can define an isomorphism of rings from $f:\textup{M}_{\mathbf{2}<\sqcup \mathbf{2}<}(P)\rightarrow \textup{M}_{\mathbf{2}<}(P)\times \textup{M}_{\mathbf{2}<}(P)$ as follows:
$$\left(\begin{array}{cccc}
        A_{0,0} & A_{0,1} & 0 & 0 \\
        0 & A_{1,1} & 0 & 0 \\
    0 & 0 & A_{3,3} & A_{3,4} \\
        0 & 0 & 0 & A_{4,4}
\end{array}\right)\mapsto \left(\begin{array}{cc}
        A_{0,0} & A_{0,1} \\
        0 & A_{1,1} 
\end{array}\right)\times \left(\begin{array}{cc}
    A_{0',0'} & A_{0',1'} \\
        0 & A_{1',1'}
\end{array}\right).$$

%\begin{coro}\label{Prop: prodiscrete ring actual result}
%Let $P$ a profinite/prodiscrete ring and $\Lambda$ an irreducible proset with . Then $\textup{M}_\Lambda(P)$ is also profinite/prodiscrete.
%\end{coro}

%\begin{proof}
%Follows from the fact that products and inverse limits of profinite/prodiscrete rings are also profinite/prodiscrete.
%\end{proof}


\subsection{Topological structure}
We now use Theorem \ref{Prop: prodiscrete ring} and Proposition \ref{prop:disjoint union and product rings} to prove properties of the rings as topological spaces. Given $P$ a topological ring,\ $\Lambda$ a proset and $S\subset P$ a non-empty subset such that $0\in S$,\ we define $$\textup{M}_\Lambda(S):=\left\{ A\in \textup{M}_\Lambda(P):\ A_{s_1,s_2}\in S \text{ for all }s_1,\ s_2\in \Lambda \right\}\subset \textup{M}_\Lambda(P).$$
\begin{remark}\label{remark:nets and open}
    Let $\{X_i\}_{i\in I}$ be a collection of topological spaces. Define $X=\prod_{i\in I}X_i$ a topological space given by the product topology on the sets $X_i$. For each $i\in I$,\ let $\pi_i:X\rightarrow X_i$ be the projection on the $i$-th coordinate. Then:
    \begin{itemize}
        \item The subsets $O\subset X$ such that for all $i\in I$ the set $\pi_i(O)$ is an open subset of $X_i$,\ and there is a finite subset $J\subset I$ such that if $i\in I\backslash J$ then $\pi_i(O)=X_i$ form a basis of open subsets of $\prod_{i\in I}X_i$.
        %\item $C\subset X$,\ $C\neq \emptyset$ is closed if,\ and only if,\ $C=\prod_{i\in I}C_i$,\ and for all $i\in I$ $C_i\neq \emptyset$ is closed in $X_i$.
        \item Given $\{x_a\}_{a\in A}$ a net in $X$ converges,\ it converges to $x$ if,\ and only if,\ for every $i\in I$ the net $\{\pi_i(x_a)\}_{a\in A}$ converges to $\pi_i(x)$ in $X_i$. 
    \end{itemize}
\end{remark}
The following results follow directly from Remark \ref{remark:nets and open} and the topology given on $\textup{M}_\Lambda(P)$ as a topological subspace of $P^{\Lambda\times \Lambda}$.

\begin{coro}\label{coro:classifying basis}
Let $P$ be a topological ring,\ $\{S_\sigma\}_{\sigma\in\Sigma}$ a basis of the neighbourhood of $0$ and $\Lambda$ a locally proset. Then $\{I^\Lambda_{\alpha}(P)+\textup{M}_\Lambda(S_\sigma)\}_{\alpha\in \Gamma(\Lambda),\ \sigma\in\Sigma}$ is a basis of the neighbourhood of $0$ in $\textup{M}_\Lambda(P)$.
\end{coro}


\begin{coro}\label{coro:open iff matrices}
Let $P$ be a topological ring and $\Lambda$ a locally finite proset. Given $J$ a two-sided open ideal of $P$ and $\{\Lambda_i\}_{i\in I}\subset \Lambda$ locally convex,\ then the following are true:
\begin{enumerate}
    \item The ideals $I^{\Lambda}_{\{\Lambda_i\}_{i\in I}}$ and $\textup{M}_\Lambda(J)$ are closed in $\textup{M}_\Lambda(P)$.
    \item The ideal $I^\Lambda_{\{\Lambda_i\}_{i\in I}}$ is open if,\ and only if,\ $\bigsqcup_{i\in I}\Lambda_i$ is finite and $P$ has the discrete topology.
    \item The ideal $\textup{M}_\Lambda(J)$ is open if,\ and only if,\ $\Lambda$ is finite.
\end{enumerate}
\end{coro}

\begin{coro}\label{coro:nets in these rings}
Let $P$ be a topological ring,\ $\Lambda$ an irreducible proset and $\{A^{(i)}\}_{i\in I}\subset \textup{M}_\Lambda(P)$ a net. The net is convergent if,\ and only if,\ for every $\alpha\in\Gamma(\Lambda)$ we have that $\{\pi_{\alpha}(A^{(i)})\}_{i\in I}$ is convergent,\ and the sequence congerges to $A$ defined coordinate-wise as follows:
$$A_{s_0,t_0}:=\left\{\begin{array}{ll}
     \lim_{i\in I}A^{(i)}_{s_0,t_0},\ &  \mbox{if } s_0  \preceq t_0\in \Lambda \\
     0,\ &  \mbox{otherwise.}
 \end{array}
\right.$$
\end{coro}




We can also easily describe a dense subset:

%\begin{proof}
%$1.$ To show they are closed note that $\textup{M}_\Lambda(J)=\bigcap_{\alpha\in \Gamma(\Lambda)}I^\Lambda_{\alpha}(P)+\textup{M}_\Lambda(J)$,\ that is,\ it is an intersection of clopen ideals hence it is closed. In a similar way,\ let $\{J_\sigma\}_{\sigma\in \Sigma}$ be a collection of two sided ideals of $P$ such that $\bigcap_{\sigma\in\Sigma}J_{\sigma}=\{0\}$ and note that $I^S_{S'}=\bigcap_{\sigma\in\Sigma} (I^S_{S'}+\textup{M}_\Lambda(J_\sigma))$.\\
%$2.$ and $3.$ follow trivially from the fact that two-sided ideals of a ring are open if,\ and only if,\ the quotient is a discrete ring and that $\textup{M}_{\bigsqcup_{i\in I}\Lambda_i}(P)$ is discrete if,\ and only if,\ $P$ is discrete and $\bigsqcup_{i\in I}\Lambda_i$ is finite.  
%\end{proof}

\begin{notation}\label{defi:dense subset}
Given $P$ a ring and $\Lambda$ a proset,\ we denote the following elements from $\textup{M}_\Lambda(P)$ as:
\begin{itemize}
    \item For $p\in P$ we define the element $p^{\Lambda}$ coordinatewise as: $$p^{\Lambda}_{s_1,s_2}:=\left\{\begin{array}{ll}
     p,\ &  \mbox{if } s_1=s_2\in \Lambda \\
     0,\ &  \mbox{otherwise.}
 \end{array}\right.$$
    \item For $S\subset \Lambda$ a subset we define the element $1^{S}$ coordinatewise as: $$1^{S}_{s_1,s_2}:=\left\{\begin{array}{ll}
     1,\ &  \mbox{if } s_1=s_2\in S \\
     0,\ &  \mbox{otherwise.}
 \end{array}\right.$$
    \item For $t_1  \preceq t_2\in \Lambda$ we define the element $e^{(t_1,t_2)}$ coordinatewise as: $$e^{(t_1,t_2)}_{s_1,s_2}:=\left\{\begin{array}{ll}
     1,\ &  \mbox{if } s_1=t_1 \text{ and }s_2=t_2 \\
     0,\ &  \mbox{otherwise.}
 \end{array}\right.$$ 
\end{itemize}
\end{notation}

Notice that for every $s\in \Lambda$,\ by definition,\ $e^{(s,s)}=1^{\{s\}}$. Given $P$ a ring and $S\subset P$ a subset we will define $\langle S\rangle$ the minimal subring of $P$ containing $S$.


\begin{prop}\label{prop:dense subset rings}
Let $P$ be a topological ring,\ $S\subset P$ a dense subset of $P$ and $\Lambda$ a proset. Then $$\textup{M}_\Lambda(P)=\overline{\langle \{p^{\Lambda}\}_{p\in S},\ \{1^{\{t\}}\}_{t\in \Lambda},\ \{e^{(s_1,s_2)}\}_{s_1  \precnapprox_2\in\Lambda} \rangle}=\overline{\langle \{p^{\Lambda}\}_{p\in S},\ \{e^{(s_1,s_2)}\}_{s_1  \preceq s_2\in\Lambda} \rangle}.$$
\end{prop}

\begin{proof}
Define $R:= \langle \{p^{\Lambda}\}_{p\in S},\ \{1^{\{t\}}\}_{t\in \Lambda},\ \{e^{(s_1,s_2)}\}_{s_1  \preceq s_2\in\Lambda} \rangle$ and $\overline{R}$ the closure of $R$ in $\textup{M}_\Lambda(P)$. Because $S\subset P$ is dense it is clear that $\{p^{\Lambda}\}_{p\in P}\subset \overline{R}$,\ hence we can use these elements to write our convergent nets.\\
\indent This result is clearly true for $\Lambda$ finite,\ as the subring $R$ contains all the elements with finitely many non-zero coordinates. Assume $\Lambda$ is infinite and let $\Gamma(\Lambda)$ be as in Theorem \ref{Prop: prodiscrete ring}. For each $\alpha\in \Gamma(\Lambda)$ define 
$$A^{(\alpha)}_{s_1,s_2}:=\left\{\begin{array}{ll}
     A_{s_1,s_2},\ &  \mbox{if } s_1,\ s_2\in\alpha \\
     0,\ &  \mbox{otherwise.}
 \end{array}\right.$$
 It is clear that these are all in $R$. By Corollary \ref{coro:nets in these rings} it follows that this net is convergent and it converges to $A$. Hence $\overline{R}=\textup{M}_{\Lambda}(P)$.
\end{proof}




\begin{coro}
Let $\Lambda$ be a proset and $P$ a topological ring. Then $\textup{M}_\Lambda(P)$ is second countable if,\ and only if,\ $P$ is second countable and $\Lambda$ is countable.
\end{coro}

\begin{proof}
If $P$ is second countable then there is $S\subset P$ a countable dense subset. By Proposition \ref{prop:dense subset rings} it follows that the set $\langle \{p^{\Lambda}\}_{p\in S},\ \{1^{\{t\}}\}_{t\in \Lambda},\ \{e^{(s_1,s_2)}\}_{s_1  \preceq s_2\in\Lambda} \rangle$ is dense in $\textup{M}_\Lambda(P)$. Because $S$ and $\Lambda$ are countable it follows that the dense subring $\langle \{p^{\Lambda}\}_{p\in S},\ \{1^{\{t\}}\}_{t\in \Lambda},\ \{e^{(s_1,s_2)}\}_{s_1  \preceq s_2\in\Lambda} \rangle$ is also countable,\ hence $\textup{M}_\Lambda(P)$ is also second countable.\\
\indent For the other side,\ notice that $\{A\in \textup{M}_\Lambda(P):\ \text{if } s_1\neq s_2\text{ then } A_{s_1,s_2}=0\}\cong\prod_{s\in \Lambda} P$ is a closed subring of $\textup{M}_\Lambda(P)$,\ and this subring is second countable if,\ and only if,\ $P$ is second countable and $\Lambda$ is countable.
\end{proof}

\subsection{Isomorphism problems for matrix rings over posets}
In this section we assume that our ordered sets are partially ordered sets and that $P$ has only $0$ and $1$ as its idempotents. The topology given to $P$ is the discrete topology.\\
\indent In this section we give conditions on the ring $P$ so two incidence rings are isomorphic if,\ and only if,\ their partially ordered sets are isomorphic. For our proofs, we will use the idempotents of our topological incidence rings to recreate the structure of our poset,\ proving that if there is an isomorphism of matrix rings,\ their posets are isomorphic as well. For that,\ first we will write down some relations between the generators of $\textup{M}_{\Lambda}$ that follow easily from the definitions, and use such properties to defined our equivalence classes of idempotents. An alternative proof of this result using Jacobison radical is given at \cite[Theorem 1]{Matrices1980}.


\begin{remark}\label{remark:relations among generators}\label{remark:order doesnt matter matrices}
Given $\Lambda$ a proset and $P$ a topological ring note that:
\begin{itemize}
    \item For every $s_1\leqslant s_2\in \Lambda$,\ $t_1\leqslant t_2\in \Lambda$
        $$e^{(s_1,s_2)}e^{(t_1,t_2)}=\left\{\begin{array}{ll}
                                        e^{(s_1,t_2)} &  \mbox{if }s_2=t_1 \\
                                        0 & \mbox{otherwise.}
                                    \end{array}\right.$$
    \item For every $s\in \Lambda$,\ 
    $$e^{(s,s)}=1^{\{s\}}.$$
    \item For every $S_1,\ S_2$ subsets of $\Lambda$                                  $$1^{S_1}1^{S_2}=\left\{\begin{array}{ll}
                                        1^{S_1\cap S_2} &  \mbox{if }S_1\cap S_2\neq\emptyset \\
                                        0 & \mbox{otherwise.}
                                    \end{array}\right.$$
                                    .
    \item For every $S\subset \Lambda$,\ $s_1\leqslant s_2 \in\Lambda$
        $$1^{S}e^{(s_1,s_2)}=\left\{\begin{array}{ll}
                                        e^{(s_1,s_2)} &  \mbox{if }s_1\in S \\
                                        0 & \mbox{otherwise.}
                                    \end{array}\right.$$
        $$e^{(s_1,s_2)}1^{S}=\left\{\begin{array}{ll}
                                        e^{(s_1,s_2)} &  \mbox{if }s_2\in S \\
                                        0 & \mbox{otherwise.}
                                    \end{array}\right.$$
    \item For every $S\subset \Lambda$,\ $p\in P$
    $$p^{\Lambda}1^{S}=1^{S}p^{\Lambda}.$$ 
    \item For every $s_1\leqslant s_2\in \Lambda$,\ $p\in P$
    $$p^{\Lambda}e^{(s_1,s_2)}=e^{(s_1,s_2)}p^{\Lambda}.$$ 
    \item Given $s,s_1,s_2\in \Lambda$ and $A\in \textup{M}_\Lambda(P)$,\ then
 $$(1^{\{s\}}A)_{t_1,t_2}=\left\{\begin{array}{ll}
     A_{t_1,t_2},\ &  \mbox{if } t_1=s  \\
     0,\ &  \mbox{otherwise.}
 \end{array}\right. $$
 $$(A1^{\{s\}})_{t_1,t_2}=\left\{\begin{array}{ll}
     A_{t_1,t_2},\ &  \mbox{if }t_2=s \\
     0,\ &  \mbox{otherwise.}
 \end{array}\right.$$
$$(1^{\{s_1\}}A1^{\{s_2\}})_{t_1,t_2}=\left\{\begin{array}{ll}
     A_{t_1,t_2},\ &  \mbox{if } t_1=s_1 \text{ and } t_2=s_2 \\
     0,\ &  \mbox{otherwise.}
 \end{array}\right. $$
 $$(A1^{\{s\}}A)_{t_1,t_2}=\left\{\begin{array}{ll}
     A_{t_1,s}A_{s,t_2},\ &  \mbox{if }s\in [t_1,\ t_2] \\
     0,\ &  \mbox{otherwise.}
 \end{array}\right.$$
\end{itemize}
These all can be proven by expanding the sums in each coordinate $(t_1,\ t_2)$.
\end{remark}

\indent We will denote 
$$\mathcal{B}(P):=\{a\in P:\ a^2=a\}$$ 
the \textbf{set of idempotents of $P$}\index{$\mathcal{B}(P)$|ndx},\ also known as the Boolean ring of $P$. This set will be given a poset structure by defining $a\leqslant b\in \mathcal{B}(P)$ if,\ and only if,\ $ab=ba=a$. Note that under this order $1$ is the maximum element and $0$ is the minimum element. \\
\indent Given $\Lambda$ a poset and $P$ a ring and,\ given $S\subset \Lambda$,\ the elements $1^{S}$ as defined in Notation \ref{defi:dense subset} are all idempotents. The following will be used throughout the whole section:

 
\begin{lemma}\label{prop:non-zero idempotent has non-zero diagonal}
Let $P$ be a ring such that $\mathcal{B}(P)=\{0,\ 1\}$,\ $\Lambda$ a poset and $A\in\mathcal{B}(\textup{M}_{\Lambda}(P))$. Then for every $s\in \Lambda$ we have $A_{s,s}\in \{0,\ 1\}$. If $A_{s,s}=0$ for every $s\in \Lambda$ then $A=0$.
\end{lemma}
 
 \begin{proof}
If $A$ is idempotent then $(A^2)_{s,s}=(A_{s,s})^2=A_{s,s}$ for every $s\in \Lambda$,\ hence $A_{s,s}\in\mathcal{B}(P)=\{0,1\}$.\\
 \indent Assume $A\in \mathcal{B}(\textup{M}_{\Lambda}(P))$ is such that $A_{s,s}=0$ for all $s\in \Lambda$. Let $s_1\leqslant s_2$. As $A^2=A$ it follows that $\sum_{t\in[s_1,s_2]}A_{s_1,t}A_{t,s_2}=A_{s_1,s_2}$. If $|[s_1,s_2]|=2$ this implies that $A_{s_1,s_2}=0$. An induction under $|[s_1,s_2]|$ with the fact all intervals are finite implies $A_{s_1,s_2}=0$,\ for every $s_1\leqslant s_2$. Hence $A=0$. 
 \end{proof}
 
\begin{lemma}\label{prop:decreasing number of diagonals}
Let $P$ be a ring such that $\mathcal{B}(P)=\{0,\ 1\}$,\ $\Lambda$ a poset and $A\in\mathcal{B}(\textup{M}_{\Lambda}(P))\backslash \{0\}$. If $s\in \{s\in \Lambda:\ \pi_{[s,s]}(A)=1\}$ then $A-A1^{\{s\}}A\in \mathcal{B}(\textup{M}_{\Lambda}(P))$ and $A-A1^{\{s\}}A< A$.
\end{lemma}

\begin{proof}
To show $A-A1^{s}A$ is an idempotent,\ notice that $$(A-A1^{\{s\}}A)^2=A^2-A^21^{\{s\}}A-A1^{\{s\}}A^2-A1^{\{s\}}A^21^{\{s\}}A=A-2A1^{\{s\}}A+A1^{\{s\}}A1^{\{s\}}A.$$ 
By Remark \ref{remark:order doesnt matter matrices},\ $1^{\{s\}}A1^{\{s\}}=1^{\{s\}}$ 
hence 
$(A-A1^{\{s\}}A)^2=A-A1^{\{s\}}A.$ \\
\indent We have that $$A(A-A1^{\{s\}}A)=A^2-A^21^{\{s\}}A=A-A1^{\{s\}}A=A^2-A1^{\{s\}}A^2=(A-A1^{\{s\}}A)A.$$
Then $A-A1^{\{s\}}A\leqslant A$.\\
\indent To show it is not an equality,\ assume that $A=A-A1^{\{s\}}A$. It follows that $A1^{\{s\}}A=0$. By Remark \ref{remark:relations among generators} this is true if,\ and only if,\ $A_{s,s}=0$,\ a contradiction to our assumption.
\end{proof}

\begin{notation}
We now define,\ for $A\in\mathcal{B}(\textup{M}_{\Lambda}(P))$,\ the set 
$$b(A)=\{s\in \Lambda:\ \pi_{[s,s]}(A)=1\}.$$
Lemma \ref{prop:decreasing number of diagonals} shows that if $A$ is a non-zero idempotent,\ then this $b(A)$ is non-empty.
\end{notation}
\indent Given a non-zero element $A\in \mathcal{B}(\textup{M}_{\Lambda}(P))$ this result gives us a way to erase one of the diagonal elements in $A$ and get an element strictly less than it under the idempotent order. We want to show that the partial order on the idempotents of $\textup{M}_{\Lambda}(P)$ is similar to the partial order on the power set of $\Lambda$ with subset order.\\

\begin{notation}
Let $P$ be a ring and $\Lambda$ a locally finite poset. Let $A\in \textup{M}_{\Lambda}(P)$ and $S\subset b(A)$ be a finite subset. We define the following:
\begin{itemize}
    \item If $S=\{s_1\}$ we define
    $$A^S=A-A1^{\{s_1\}}A.$$
    \item If $A^S$ was defined for $S=\{s_1,\ \ldots,\ s_{n-1}\}$, and $s_n\in b(A)\backslash S$, we define 
    $$A^{S\cup \{s_n\}}=A^{S}-A^S 1^{\{s_n\}}A^S.$$
\end{itemize}
\end{notation}

\begin{lemma}\label{lemma:above}
Let $\Lambda$ be a poset and $P$ be a ring such that $\mathcal{B}(P)=\{0,\ 1\}$. Let $A\in\mathcal{B}(\textup{M}_\Lambda(P))$ such that $b(A)$ has at least two elements. Let $s_1\neq s_2\in b(A)$. Then $A^{\{s_1,s_2\}}=A^{\{s_2,s_1\}}$.
\end{lemma}

\begin{proof}
We have that 
$$A^{\{s_1,s_2\}}=A-A1^{\{s_1\}}A-A1^{\{s_2\}}A+A1^{\{s_1\}}A1^{\{s_2\}}A+A1^{\{s_2\}}A1^{\{s_1\}}A-A1^{\{s_1\}}A1^{\{s_2\}}A1^{\{s_1\}}A$$
$$A^{\{s_2,s_1\}}=A-A1^{\{s_2\}}A-A1^{\{s_1\}}A+A1^{\{s_2\}}A1^{\{s_1\}}A+A1^{\{s_1\}}A1^{\{s_2\}}A-A1^{\{s_2\}}A1^{\{s_1\}}A1^{\{s_2\}}A$$
By Remark \ref{remark:order doesnt matter matrices},\ we get that $1^{\{s_1\}}A1^{\{s_2\}}A1^{\{s_1\}}=1^{\{s_2\}}A1^{\{s_1\}}A1^{\{s_2\}}=0$. Hence $A^{\{s_1,s_2\}}=A^{\{s_2,s_1\}}$.
\end{proof}

It follows that for every finite set $S$ the construction of $A^S$ does not depend on the order of $S$. We can then define $A^S$ for the case $S$ is infinite as follows:\\
\indent If $S$ is infinite,\ let $I=\{S'\subset S:\ S'\text{ is finite}\}$ with order given by containment. Define $A^S$ as the limit of the net $\{A^{S'}\}_{S'\in I}$,\ that is,\ $$A^S=\lim_{S'\in I}A^{S'}.$$
This limit is well-defined as $P$ has the discrete topology. By Corollary \ref{coro:nets in these rings} this net is convergent. By Lemma \ref{lemma:above},\ the definition of $A^S$ also doesn't depend on the ordering of $S$ even in the case $S$ is infinite,\ hence $A^S$ is uniquely defined. Proposition \ref{prop:decreasing number of diagonals} implies the element $A^S$ is an idempotent.

\begin{theorem}\label{thrm:one non-zero diagonal matrices}
Let $P$ be a ring such that $\mathcal{B}(P)=\{0,\ 1\}$,\ $\Lambda$ a poset and $A\in\mathcal{B}(\textup{M}_{\Lambda}(P))\backslash \{0\}$. Given $S\subset b(A)$ a non-empty subset,\ then $A^{S}< A$ and $A^{S}_{s,s}=1$ if,\ and only if,\ $s\in b(A)\backslash S$. More than that,\ if $S_1\subset S_2\subset b(A)$ then $A^{S_2}\leqslant A^{S_1}$ with equality if,\ and only if,\ $S_1=S_2$.
\end{theorem}

\begin{proof}
The proof for the finite case follows directly from the definition and Lemma \ref{prop:decreasing number of diagonals}.\\
\indent By the definition of the net and the idempotent order it clear that,\ for all $S'\subset S$ finite subsets,\ $AA^{S'}=A^{S'}A=A^{S'}$. Hence $A^{S}A=\lim AA^{S'}=\lim A^{S'}A=\lim A^{S'}=A^{S}$. We then proved the first part of the statement.\\
\indent For the second part,\ let $S_1\subset S_2\subset b(A)$. The result is trivial for the case $S_1$ is finite,\ hence we assume $S_1$ is infinite. Then $$A^{S_1}A^{S_2}=\lim_{S'_1\subset_{\text{finite}} S_1}A^{S'_1}A^{S_2}=\lim_{S'_1\subset_{\text{finite}} S_1}A^{S_2}A^{S'_1}=A^{S_2},$$
hence $A^{S_2}\leqslant A^{S_1}$. If $S_1\neq S_2$,\ then given $s\in S_2\backslash S_1$,\ by Lemma \ref{prop:decreasing number of diagonals},we have that $A^{S_2}\leqslant A^{S_1\cup \{s\}}< A^{S_1}$,\ that is,\ $A^{S_1}\neq A^{S_2}$.

\end{proof}

\begin{coro}
Let $\Lambda$ be a poset and $P$ a ring such that $\mathcal{B}(P)=\{0,\ 1\}$. If $A\in \mathcal{B}(\textup{M}_{\Lambda}(P))\backslash\{0\}$ is such that $A$ has only one non-zero diagonal coordinate,\ say $A_{s,s}=1$,\ then $A-A1^{(s)}A=0$.
\end{coro}


The initial idea from this section is using idempotents of the form $1^{\{s\}}$ to recover our poset structure. The problem is that isomorphirms don't necessarily send elements with only one non-zero coordinate to other elements with only one non-zero coordinate. Following is an example for $2\times 2$ triangular matrices:

$$\left(\begin{array}{ll}
1 & a \\
0 & 1
\end{array}\right) \cdot\left(\begin{array}{ll}
1 & 0 \\
0 & 0
\end{array}\right) \cdot\left(\begin{array}{ll}
1 & a \\
0 & 1
\end{array}\right)^{-1}=\left(\begin{array}{cc}
1 & -a \\
0 & 0
\end{array}\right)$$

The next few definitions will be central to tackle such problem:

\begin{defi}[Definition 86.4.8 \cite{stacks-project}]\index{topologically nilpotent|ndx}
Let $P$ be a topological ring. We say an element $r\in P$ is \textbf{topologically nilpotent} if $\lim_{n\in\mathbb{N}}r^n=0$.
\end{defi}

In \cite{stacks-project} the notion of topologically nilpotent is given for topological rings with a neighbourhood of $0$ consisting of ideals,\ known as linearly topologized \cite[Definition 15.36.1]{stacks-project}. As our rings might not be linearly topologized,\ we define topologically nilpotent in a more general way. 

\begin{ex}
\begin{itemize}
    \item Given $\mathbb{R}$ the ring of real numbers with the usual topology,\ for all $r\in (-1,\ 1)$ we have that $r$ is topologically nilpotent.
    \item Given $\mathbb{Z}_p$ the p-adic integers,\ then for all $r\in p\mathbb{Z}_p$ we have that $r$ is topologically nilpotent.
    \item Let $P$ a topological ring and $\Lambda$ a poset. If $A\in \textup{M}_{\Lambda}(P)$ is such that for all $s\in \Lambda$,\ $A_{s,s}=0$,\ then $A$ is topologically nilpotent. Notice that if $|[s_1,\ s_2]|=2$ then $$(A^2)_{s_1,s_2}=A_{s_1,s_1}A_{s_1,s_2}+A_{s_1,s_2}A_{s_2,s_2}=0.$$
    In general,\ the poset structure on $\Lambda$ implies that if $|[s_1,\ s_2]|=n$ then $(A^n)_{s_1,s_2}=0$. This fact can easily be proved by induction. Corollary \ref{coro:nets in these rings} then implies such $A$ is topologically nilpotent.
\end{itemize}
\end{ex}

%%\begin{lemma}
%%Given $\Lambda$ a poset and $P$ a ring,\ an element $A\in \textup{M}_{\Lambda,P)$. If $A$ is topologically nilpotent then for every $s\in \Lambda$ we have $A_{s,s}$ is topologically nilpotent.
%%\end{lemma}

%%\begin{proof}
%%Let $A$ be topologically nilpotent. The fact that $A_{s,s}$ is topologically nilpotent,\ for every $s\in\Lambda$ follows from $(A^n)_{s,s}=(A_{s,s})^n$ for every $s\in \Lambda$.
%%\end{proof}

The following two definitions will allow us to order the idempotents of $\textup{M}_{\Lambda}(P)$ in such a way we can recover the poset structure of $\Lambda$ from the ring of matrices.

\begin{defi}
Let $P$ be a topological ring with only $0$ and  $1$ as its idempotents and $\Lambda$ a poset. We define an relation $\sim$ in $\mathcal{B}(\textup{M}_{\Lambda}(P))$ as $A\sim B$ if,\ and only if,\ $A-B$ is topologically nilpotent. The equivalence class of an idempotent $A\in\mathcal{B}(P)$ is denoted as $[A]$.
\end{defi}


\begin{defi}\index{minimal non-zero|ndx}
Let $\Lambda$ be a poset. Given that $\Lambda$ has $0$ a minimum element,\ we say $s\in \Lambda$ is \textbf{minimal non-zero} if $[0,\ s]=\{0,\ s\}$,\ that is,\ there is no element $t\in \Lambda$ such that $0<t$ and $t<s$.
\end{defi}

\begin{lemma}\label{lemma:properties of equiv relation idenpot}
Let $\Lambda$ be a poset and $P$ a ring such that $\mathcal{B}(P)=\{0,\ 1\}$. The following are true for the relation $\sim$ in $\textup{M}_{\Lambda}(P)$:
\begin{enumerate}
    \item $A\sim B$ in $\mathcal{B}(\textup{M}_{\Lambda(P)})$ if,\ and only if,\ $b(A)=b(B)$.
    \item It is an equivalence relation.
    \item For every $A\in \mathcal{B}(\textup{M}_{\Lambda}(P))$ there exists an unique $S\subset \Lambda$ such that $A\sim 1^{S}$.
    \item Given $[A],\ [B]$ equivalence classes,\ the order given by $[A]\leqslant[B]$ if there are $A\in [A]$,\ $B\in [B]$ such that $A\leqslant B$ in relation to the idempotent order is a partial order.
    \item There is an order preserving bijection from the power set of $\Lambda$ and the equivalence classes of idempotents $\mathcal{B}(\textup{M}_{\Lambda}(P))$. The elements of $\Lambda$ can be identified with the minimal non-zero elements of $\mathcal{B}(\textup{M}_{\Lambda}(P))$.
\end{enumerate}
\end{lemma}

\begin{proof}
$\mathit{1.}$ Let $A,\ B\in \mathcal{B}(\textup{M}_{\Lambda}(P))$. Notice that if $b(A)\neq b(B)$,\ there is $t\in \Lambda$ such that $(A-B)_{s,s}\in \{1,\ -1\}$. Theorem \ref{thrm:one non-zero diagonal matrices} then implies that $A-B$ is not topologically nilpotent. On the other hand,\ if $b(A)=b(B)$ by Theorem \ref{thrm:one non-zero diagonal matrices} and Lemma \ref{prop:non-zero idempotent has non-zero diagonal} we have that $A-B$ is topologically nilpotent,\ proving the argument.\\
\indent Statement $\mathit{2.}$ and $\mathit{3.}$ follows directly from $\mathit{1.}$, and statements $\mathit{4.}$ and $\mathit{5.}$ follows directly from $\mathit{3}$.
\end{proof}

\begin{ex}\label{ex:problemo} 
    Notice that for the case $\Lambda$ is a proset this is not necessarily an equivalence relation on $\textup{M}_\Lambda(P)$. For example,\ on the case $\Lambda=\mathbf{2}$ and $P=\mathbb{Z}_p$ we have that
$$\left(\begin{array}{cc}
        1 & p \\
        0 & 0 
\end{array}\right)-\left(\begin{array}{cc}
        1 & 0 \\
        p & 0 
\end{array}\right)=\left(\begin{array}{cc}
        0 & p \\
        -p & 0 
\end{array}\right)$$
and 
$$\left(\begin{array}{cc}
        0 & p \\
        -p & 0 
\end{array}\right)^{2n}=\left(\begin{array}{cc}
        (-1)^{n}p^{2n} & 0 \\
        0 & (-1)^{n}p^{2n} 
\end{array}\right)\xrightarrow{n\rightarrow \infty} \left(\begin{array}{cc}
        0 & 0 \\
        0 & 0 
\end{array}\right)$$
$$\left(\begin{array}{cc}
        0 & p \\
        -p & 0 
\end{array}\right)^{2n+1}=\left(\begin{array}{cc}
        0 & (-1)^{n}p^{2n+1} \\
        -(-1)^{n}p^{2n+1} & 0 
\end{array}\right)\xrightarrow{n\rightarrow \infty} \left(\begin{array}{cc}
        0 & 0 \\
        0 & 0 
\end{array}\right)$$
hence it is topologically nilpotent. It is also the case that
$$\left(\begin{array}{cc}
        1 & p \\
        0 & 0 
\end{array}\right)-\left(\begin{array}{cc}
        1 & 1 \\
        0 & 0 
\end{array}\right)=\left(\begin{array}{cc}
        0 & p-1 \\
        0 & 0 
\end{array}\right)$$
$$\left(\begin{array}{cc}
        1 & 0 \\
        p & 0 
\end{array}\right)-\left(\begin{array}{cc}
        1 & 0 \\
        1 & 0 
\end{array}\right)=\left(\begin{array}{cc}
        0 & 0 \\
        p-1 & 0 
\end{array}\right)$$
are nilpotent,\ hence topologically nilpotent. But
$$\left(\left(\begin{array}{cc}
        1 & 1 \\
        0 & 0 
\end{array}\right)-\left(\begin{array}{cc}
        1 & 0 \\
        1 & 0 
\end{array}\right)\right)^{2n}=\left(\begin{array}{cc}
        (-1)^n & 0 \\
        0 & (-1)^n 
\end{array}\right)$$
is not topologically nilpotent.

\end{ex}

%\subsection{Recovering the poset structure}

\begin{lemma}\label{prop:rewriting A' for minimal non-zero}
Let $P$ be a ring such that $\mathcal{B}(P)=\{0,\ 1\}$ and $\Lambda$ a poset. Given $A\in\mathcal{B}(\textup{M}_\Lambda(P))\backslash \{0\}$ idempotent,\ then $A=1^{S}+A'$ for some $S\subset \Lambda$,\ $A'$ topologically nilpotent with $A'_{s,s}=0$ for all $s\in\Lambda$. If $[A]$ is minimal non-zero then $A'=1^{\{s\}}A'+A'1^{\{s\}}+A'1^{\{s\}}A'$.
\end{lemma}

\begin{proof}
Because $A\in \mathcal{B}(\textup{M}_\Lambda(P))\backslash\{0\}$ then,\ by Lemma \ref{lemma:properties of equiv relation idenpot},\ there is $S\subset \Lambda$ such that $A\sim 1^S$. Hence,\ by definition of the equivalence relation,\ $A-1^S=A'$ for $A'$ topologically nilpotent. Then $A=1^S+A'$,\ where $A'_{s,s}=0$ for all $s\in\Lambda$. \\
\indent If $[A]$ is minimal non-zero then there is $s\in \Lambda$ such that $[A]=[1^{\{s\}}]$. By Lemmas \ref{prop:decreasing number of diagonals} and \ref{prop:non-zero idempotent has non-zero diagonal},\ $A-A1^{\{s\}}A=0$. We can write $A$ as $1^{\{s\}}+A'$,\ as shown above. Using the property $A$ is an idempotent we get $$(1^{\{s\}}+A')^2=1^{\{s\}}+1^{\{s\}}A'+A'1^{\{s\}}+A'1^{\{s\}}A'=1^{\{s\}}+A'.$$
Rearranging the equation then gives us $A'=1^{\{s\}}A'+A'1^{\{s\}}+A'1^{\{s\}}A'$.
\end{proof} 

\begin{coro}\label{coro:quasiminal and intervals}
Let $A\in \mathcal{B}(\textup{M}_\Lambda(P))$ be minimal non-zero and $s\in \Lambda$ be such that $A\sim 1^{\{s\}}$. Then $A_{s_1,s_2}$ can be non-zero if,\ and only if,\ $s\in[s_1,\ s_2]$.
\end{coro}

\begin{proof}
A direct corollary from Lemma \ref{prop:rewriting A' for minimal non-zero} and from Remark \ref{remark:order doesnt matter matrices}.
\end{proof}


\begin{lemma}\label{prop:how idempotent classes are sent to other}
Let $\Lambda_1,\Lambda_2$ be two posets and $P$ a topological ring such that $\mathcal{B}(P)=\{0,\ 1\}$. If $f:\textup{M}_{\Lambda_1}(P)\rightarrow \textup{M}_{\Lambda_2}(P)$ is a continuous homomorphism of rings then,\ for every $S_1\subset \Lambda_1$ there is $S_2\subset \Lambda_2$ such that $f([1^{S_1}])\subset [1^{S_2}]$. It is also the case that if $S\subset S'\subset \Lambda$ then $[f(1^S)]\leqslant [f(1^{S'})]$.
\end{lemma}
 
\begin{proof}
Let $A\in [1^{S_1}]$. As homomorphisms send idempotents to idempotents,\ Lemma \ref{prop:rewriting A' for minimal non-zero} implies $f(A)=1^{S_2}+f(A)'$ for some $S_2\subset \Lambda_2$ and $f(A)'\in \textup{M}_{\Lambda_2}(P)$ topologically nilpotent. Hence $f(A)\in [1^{S_2}]$.\\
\indent Suppose now $B\in [1^{S_1}]$. Then $B-A$ is topologically nilpotent and,\ because $f$ is continuous,\ it follows that $f(B-A)$ is topologically nilpotent. Then $f(B)\in [f(A)]=[1^{S_2}]$ for every $B\in [1^{S_1}]$. Hence $f[1^{S_1}]\subset [f(1^{S_1})]=[1^{S_2}]$,\ for some $S_2\subset \Lambda_2$.\\
\indent For the last statement,\ assume $[1^S]< [1^{S'}]$. Hence $f(1^{S'})f(1^{S})=f(1^{S})f(1^{S'})=f((1^{S}+1^{S'\backslash S'})(1^S))=f(1^S)$,\ that is,\ $[f(1^S)]\leqslant [f(1^{S'})]$.
\end{proof} 
The next result is essential for the proof of the isomorphism problem on the rings of matrices indexed by ordered sets. It connects properties of the minimal non-zero elements and the ordering of our ordered set.

\begin{lemma}\label{prop:isomorphism problem rings}
Let $[1^{\{s_1\}}],[1^{\{s_2\}}]$ be minimal non-zero classes of $\textup{M}_\Lambda(P)$,\ for a ring $P$ such that $\mathcal{B}(P)=\{0,\ 1\}$ and $\Lambda$ a poset. Then there is $A\in [1^{\{s_1\}}]$,\ $B\in[1^{\{s_2\}}]$ such that $AB\neq 0$ if,\ and only if,\ $s_1\leqslant s_2$. It is the case $s_1=s_2$ if,\ and only if,\ $AB\neq 0$ for every $A\in [1^{\{s_1\}}]$ and $B\in[1^{\{s_2\}}]$.
\end{lemma}

\begin{proof}
Let $[1^{\{s_1\}}],\ [1^{\{s_2\}}]$ be two minimal non-zero classes and let $A\in [1^{\{s_1\}}],\ B\in [1^{\{s_2\}}]$. Write $A=1^{\{s_1\}}+A'$ and $B=1^{\{s_2\}}+B'$,\ as in Lemma \ref{prop:rewriting A' for minimal non-zero}. We first show that if $AB\neq 0$ then $s_1\leqslant s_2$. Notice that $AB$ can be written as follows
$$AB=1^{\{s_1\}}1^{\{s_2\}}+1^{\{s_1\}}B'+A'1^{\{s_2\}}+A'B'.$$
Hence,\ if $AB\neq 0$,\ at least one of the terms above is non-zero. We now work on necessary conditions for each term to be non-zero:
\begin{itemize}
    \item Remark \ref{remark:relations among generators} implies $1^{\{s_1\}}1^{\{s_2\}}\neq 0$ if,\ and only if $s_1=s_2$.
    \item By Remark \ref{remark:order doesnt matter matrices} and Corollary \ref{coro:quasiminal and intervals} we have that $1^{\{s_1\}}B'$ is non-zero if,\ and only if,\ $s_1 \leqslant s_2$ and $B'_{s_1,s_2}\neq 0$.
    \item Similar to the case $1^{\{s_1\}}B'$,\ $A'1^{\{s_2\}}$ is non-zero if,\ and only if,\ $s_1\leqslant s_2$ and $A'_{s_1,s_2}\neq 0$.
    \item For $A'B'$,\ notice that by Lemma \ref{prop:rewriting A' for minimal non-zero} we can rewrite it as: 
$$(1^{\{s_1\}}A'+A'1^{\{s_1\}}+A'1^{\{s_1\}}A')(1^{\{s_2\}}B'+B'1^{\{s_2\}}+B'1^{\{s_2\}}B').$$
After expanding,\ the terms are of the form $X1^{\{s_1\}}Y1^{\{s_2\}}Z$ for $X,Y,Z\in \{1^{\Lambda},A',B',A'B'\}$. By Remark \ref{remark:order doesnt matter matrices} if $s_1\nleqslant s_2$ then $1^{\{s_1\}}Y1^{\{s_2\}}=0$. Hence if $A'B'\neq 0$ we have $s_1\leqslant s_2$.
\end{itemize}
That is,\ if $AB\neq 0$ then $s_1\leqslant s_2$. We now need to proof the other side.\\
\indent Let $s_1\leqslant s_2$. Define the matrix $A$ coordinate-wise as follows:
$$A_{t_1,t_2}=\begin{cases}
1 & \mbox{if }t_1=t_2=s_1 \mbox{ or }t_1=s_1,\ t_2=s_2\\
0 & \mbox{otherwise.}
\end{cases}$$
By Remark \ref{remark:order doesnt matter matrices},\ $A1^{s_2}\neq 0$. Hence,\ we get the only if side.\\
\indent Now assume $s_1=s_2=s$. By Lemma \ref{prop:rewriting A' for minimal non-zero} it follows that for all $A,B\in [1^{\{s\}}]$ we have $AB=1^{\{s\}}+1^{\{s\}}B'+A'1^{\{s\}}+A'B'$. As $1^{\{s\}}B'+A'1^{\{s\}}+A'B'$ is topologically nilpotent and $1^{\{s\}}$ is not,\ we have that $AB\neq 0$.\\
\indent In the case $s_1<s_2$,\ $1^{\{s_1\}}1^{\{s_2\}}=0$. Hence there are $A\in [1^{\{s_1\}}]$,\ $B\in [1^{\{s_2\}}]$ such that $AB=0$.
\end{proof}

Now the process of rebuilding our poset using our matrices ring is as follows:
\begin{itemize}
    \item The elements of our poset will be the minimal non-zero classes of idempotents,\ which can be written as $[1^{\{s\}}]$ for $s\in \Lambda$.
    \item If there are $A\in [1^{\{s_1\}}]$ and $B\in [1^{\{s_2\}}]$ such that $AB\neq 0$ we get $s_1\leqslant s_2$. If it is also the case that there are idempotents $A\in [1^{\{s_1\}}]$ and $B\in [1^{\{s_1\}}]$ such that $AB= 0$,\ then $s_1=s_2$. 
\end{itemize}

By Lemma \ref{prop:isomorphism problem rings} it follows that the set of minimal non-zero idempotents with order as given above is the same as $\Lambda$. With Lemma \ref{prop:how idempotent classes are sent to other} we get that isomorphisms send minimal non-zero to minimal non-zero. We can then prove the following:

\begin{theorem}\cite[Theorem 1]{Matrices1980}\label{thrm:isomorphism problem of rings}
Let $\Lambda_1,\ \Lambda_2$ be posets and $P$ be a topological ring  such that $\mathcal{B}(P)=\{0,\ 1\}$. Then $\textup{M}_{\Lambda_1}(P)\cong \textup{M}_{\Lambda_2}(P)$ if,\ and only if,\ $\Lambda_1\cong \Lambda_2$,\ that is,\ there is a bijective order preserving map from $\Lambda_1$ to $\Lambda_2$.
\end{theorem}

\begin{proof}
Assume $f:\textup{M}_{\Lambda_1}(P)\rightarrow \textup{M}_{\Lambda_2}(P)$ is a continuous isomorphism. Because $f$ is a ring isomorphism,\ Lemma \ref{prop:how idempotent classes are sent to other} implies that for all $s_1\in \Lambda_1$ there exists an unique $s_2\in\Lambda_2$ such that $f([1^{\{s_1\}}])=[1^{\{s_2\}}]$,\ as these are minimal non-zero. Hence $f$ gives a bijection from $\{[1^{\{s_1\}}]:\ s_1\in\Lambda_1\}$ and $\{[1^{\{s_2\}}]:\ s_2\in\Lambda_2\}$. Notice that the continuous isomorphism of rings also preserve all the properties from Lemma \ref{prop:isomorphism problem rings}. Hence the map $\tilde{f}:\Lambda_1\rightarrow \Lambda_2$ defined by $s_1\mapsto s_2$ if,\ and only if,\ $f([1^{\{s_1\}}])= [1^{\{s_2\}}]$ is an order preserving bijective map. Hence $\Lambda_1\cong \Lambda_2$.\\
\indent On the other hand,\ let $f:\Lambda_1\rightarrow\Lambda_2$ an order preserving bijective map. It is easy to see that the map
$$\begin{array}{llll}
    \tilde{f}:& \textup{M}_{\Lambda_2}(P) &\longrightarrow &  \textup{M}_{\Lambda_1}(P) \\
     & A & \longmapsto & \tilde{f}(A)
\end{array}$$
where $\tilde{f}(A)_{s_1,s_2}=A_{f(s_1),f(s_2)}$,\ is a continuous isomorphism of rings.
\end{proof}

Theorem \ref{thrm:isomorphism problem of rings} is not always true for topological rings. In fact, \cite[Proposition 1]{Matrices1980} proves that if $\Lambda$ is a locally finite pre-ordered set then there exists $P$ a ring such that $P\cong \textup{M}_{\Lambda}(P)$. In the same article, it is also shown that if $P$ is a ring that is simple Artinian modulo the Jacobson radical and $\Lambda_1,\ \Lambda_2$ are prosets, then $\textup{M}_{\Lambda_1}(P)\cong \textup{M}_{\Lambda_2}(P)$ if, and only if, $\Lambda_1\cong \Lambda_2$. A list of answers for the isomorphism problem in different classes of incidence rings can be seen at \cite{recovery_question}.

==> Sections/4-Functor.tex <==
\section{Categorical properties}\label{categorical_properties}\label{5.4}

\subsection{The functor \texorpdfstring{$\mathbf{M}_\_(P)$}{TEXT}}

Theorem \ref{thrm:isomorphism problem of rings} closely relates the structure of matrix rings of the form $\textup{M}_\Lambda(P)$ with their respective 
partially ordered sets. In this section we will show that this can be extended to defining a contravariant functor from a category of partially ordered sets to the category of rings,\ showing that even products and inverse limits of these rings can be understood just by looking at limits and coproducts on the category or partially ordered sets. This question arise naturally from Proposition \ref{prop:disjoint union and product rings} and Theorem \ref{Prop: prodiscrete ring},\ which points to the direction that coproducts are mapped to products and colimits to limits under such map.\\
\indent For this section we will need to restrict the maps we accept for the category of ordered sets,\ as not all maps would work. We then give arguments for why each condition is added.

\begin{defi}\label{defi:morphisms of prosets/posets}\index{order preserving map|ndx}\index{convex embedding|ndx}\index{FCC map|ndx}
Given $\Lambda,\ \Lambda'$ two prosets and $f:\Lambda\rightarrow\Lambda'$ a set function. We say that:
\begin{itemize}
    \item $f$ is \textbf{order preserving} if for $a\preceq b\in \Lambda$ then $f(a)\preceq f(b)\in \Lambda'$.
    \item $f$ is a \textbf{convex function} if it is an order preserving function and whenever $\alpha\subset\Lambda$ is a convex subset then $f(\alpha)$ is a convex subset of $\Lambda'$.
    \item $f$ is a \textbf{convex embedding} if it is a convex function and injective.
    \item $f$ is \textbf{constant}\index{constant|ndx} if $f(\Lambda)=\{t\}$,\ for some $t\in\Lambda'$
    \item Given that $\sqcup_{i\in I}\Lambda_i$ is the decomposition of $\Lambda$ into its components. we say $f$ \textbf{factors out into constant functions and convex embeddings (FCC)} if for each $i\in I$ either the function $f|_{\Lambda_i}:\Lambda_i\rightarrow\Lambda'$ is a constant function or a convex embedding.
\end{itemize}
\end{defi}
Let $f:\Lambda_1\rightarrow \Lambda_2$ be an order preserving morphism. A first idea for a map $\Tilde{f}:\textup{M}_{\Lambda_1}(P)\rightarrow \textup{M}_{\Lambda_2}(P)$ is as in Theorem \ref{thrm:isomorphism problem of rings}. We then have $\Tilde{f}(A)$ is defined coordinatewise as 
$$(\Tilde{f}(A))_{s_1,s_2}=\sum A_{t_1,t_2}$$ 
for $t_1,t_2\in \Lambda_1$,\ $f(t_1)=s_1$,\ $f(t_2)=s_2$.
\begin{enumerate}
    \item If $f$ is injective,\ but not surjective,\ then $\Tilde{f}(1^{\Lambda_1})\neq 1^{\Lambda_2}$,\ hence it is not a ring homomorphism. For example:
$$f:2<\rightarrow 3<$$
$$f(0)=0,\ \ f(1)=2$$
then
$$\Tilde{f}:\textup{M}_{2<}(P)\rightarrow \textup{M}_{3<}(P)$$
$$\left(\begin{array}{cc}
   a_{0,0}  &  a_{0,1} \\
    0 & a_{1,1}
\end{array}\right)\mapsto \left(\begin{array}{ccc}
   a_{0,0}  &  0 & a_{0,1}\\
    0 & 0 & 0\\
    0 & 0 & a_{1,1}
\end{array}\right).$$
\item If $f$ is surjective,\ but not injective,\ it does not preserve multiplication. For example:
$$f:2<\rightarrow 1$$
then
$$\Tilde{f}:\textup{M}_{2<}(P)\rightarrow \textup{M}_1(P)$$
$$\left(\begin{array}{cc}
   a_{0,0}  &  a_{0,1} \\
    0 & a_{1,1}
\end{array}\right)\mapsto a_{0,0}+a_{0,1}+a_{1,1}.$$
\end{enumerate}

\noindent Hence it is necessary to make some tweaks when defining a morphism between matrix rings in relation to a morphism between prosets.\\
\indent A second idea is reversing the direction of $f:\Lambda_1\rightarrow \Lambda_2$. We can then define $\mathbf{M}[f]$ on the set of generators (Proposition \ref{prop:dense subset rings}) of $\textup{M}_{\Lambda_2}(P)$ as follows:
$$\begin{array}{llll}
    \mathbf{M}[f]:&\textup{M}_{\Lambda_2}(P) &\longrightarrow & \textup{M}_{\Lambda_1}(P)\\
     & p^{\Lambda_2} & \longmapsto & p^{\Lambda_1}\\
     & e^{(s_1,s_2)}&\longmapsto & \left\{\begin{array}{ll}
                                          \sum_{t_1,t_2}e^{(t_1,t_2)}    &  \mbox{for }t_1\preceq t_2 \mbox{ and }f(t_1)=s_1,\ f(t_2)=s_2\\
                                       0      &  \mbox{otherwise}
                                    \end{array}\right.    
\end{array}$$

 In this case we have the following:

\begin{prop}
Assume $\Lambda_1,\ \Lambda_2$ are prosets and $P$ is a ring. Let $f:\Lambda_1\rightarrow \Lambda_2$ be an order preserving morphism that is not convex. Then  $\mathbf{M}[f]$ is not well-defined.
\end{prop}

\begin{proof}
Let $f$ be an order preserving that is not convex. If $f$ is not convex then there is $\alpha\in \Lambda_1$ a convex set such that $f(\alpha)$ is not convex in $\Lambda_2$. Hence either $f(\alpha)$ is not closed under intervals or it is not connected.\\
\indent If $f(\alpha)$ is not connected,\ there are $s_1,\ s_2\in \alpha$ such that $[s_1,\ s_2]\neq \emptyset$,\ but $[f(s_1),\ f(s_2)]=\emptyset$. That is,\ $s_1\preceq s_2$ but $f(s_1)\npreceq f(s_2)$,\ a contradiction to the assumption $f$ is order preserving.\\
\indent If $f$ is not closed under intervals,\ there are $s_1\preceq s_2\in \Lambda_1$ such that $[f(s_1),\ f(s_2)]$ is not in $f(\alpha)$. Then there is $f(s_1)\precnapprox t\precnapprox f(s_2)$ such that $f^{-1}(t)=\emptyset$. In this case we then have
$$\mathbf{M}[f](e^{(f(s_1),t)})\mathbf{M}[f](e^{(t,f(s_2))})=0$$
but 
$$\mathbf{M}[f](e^{(f(s_1),f(s_2))})$$
contains $e^{(s_1,s_2)}$ as a term,\ hence is non-zero. That is,\ $$\mathbf{M}[f](e^{(f(s_1),t)})\mathbf{M}[f](e^{(t,f(s_2))})\neq \mathbf{M}[f](e^{(f(s_1),f(s_2))}).$$


%\indent If it is not connected,\ there exist .\\
%\indent Now let $s_1,s_2$ as in the claim,\ and $t\in \Lambda_2$ be such that $f(s_1)< t\precnapprox f(s_2)$. Notice that $(e^{(s_1,s_2)}+e^{(s_1,t)}+e^{(t,s_2)})^2=e^{(s_1,s_2)}$. We will show the left side and right side of the equation cannot be the same given our initial condition.\\
%\indent On one hand
%\begin{equation}\label{eq:5}
%    \mathbf{M}[f](e^{(s_1,s_2)})=\sum_{t_1,t_2} e^{(t_1,t_2)},
%\end{equation}
%for $f(t_1)=f(s_1)$,\ $f(t_2)=f(s_2)$ and $t_1\precnapproxt_2$.\\
%\indent On the other hand $\mathbf{M}[f](e^{(f(s_1),f(s_2))}+e^{(f(s_1),t)}+e^{(t,f(s_2))})=\sum_{t_1,t_2} e^{(t_1,t_2)}$,\ for $f(t_1)=f(s_1)$,\ $f(t_2)=f(s_2)$ and $t_1\precnapproxt_2$. Hence 
%\begin{equation}\label{eq:6}
%    \mathbf{M}[f](e^{(f(s_1),f(s_2))}+e^{(f(s_1),t)}+e^{(t,f(s_2))})^2=(\sum_{t_1,t_2} e^{(t_1,t_2)})^2=\sum_{q_1,q_2}e^{(q_1,q_2)}
%\end{equation}
%such that $q_1\precnapproxq_2$,\ $f(q_1)=s_1$,\ $f(q_2)=s_2$ and there exists $q_1\precnapproxq\precnapproxq_2$ such that $f(q)\in\{s_1,s_2\}$. If there is no such $q_1,q_2$ then $(\ref{eq:6})=0$. If there exists such a $q$,\ fix a $q$ such that $|[q,q_2]|=2$. Then $e^{(q,q_2)}$ is part of the sum in $(\ref{eq:5})$ but not of the sum in $(\ref{eq:6})$. In both cases $(\ref{eq:5})\neq(\ref{eq:6})$.\\
%\indent Hence $\mathbf{M}[f]((e^{(s_1,s_2)}+e^{(s_1,t)}+e^{(t,s_2)})^2)\neq (\mathbf{M}[f](e^{(s_1,s_2)}+e^{(s_1,t)}+e^{(t,s_2)}))^2$ and $\mathbf{M}[f]$ cannot be a ring homomorphism.
\end{proof}

An example of the result above is as follows: let $f:\mathbf{2}<\longrightarrow \mathbf{3}<$ defined by $f(0)=0$,\ $f(1)=2$. This map is order preserving but not convex. The $\mathbf{M}[f]:{M}_{\mathbf{3}<}(P)\rightarrow {M}_{\mathbf{2}<}(P)$ would be defined as follows:
$$ \left(\begin{array}{lll}
a_{0,0} & a_{0,1} & a_{0,2} \\
0 & a_{1,1} & a_{1,2} \\
0 & 0 & a_{2,2} 
\end{array}\right) \mapsto \left(\begin{array}{ll}
a_{0,0} & a_{0,2} \\
0 & a_{2,2} 
\end{array}\right) $$
which is easily seen not to preserve multiplication. \\
\indent It is still not known if it the morphism being FCC is a necessary condition for $\mathbf{M}[f]$ to be well-defined,\ but there are some examples showing that being convex is not sufficient. For instance,\ let  $f:\mathbf{4<}\rightarrow\mathbf{2<}$ defined as $f(0)=f(1)=0$,\ $f(2)=f(3)=1$. The map $\mathbf{M}[f]:{M}_{\mathbf{2}<}(P)\rightarrow {M}_{\mathbf{4}<}(P)$ would be defined as follows:
$$ \left(\begin{array}{ll}
a_{0,0} & a_{0,1} \\
0 & a_{1,1} 
\end{array}\right) \mapsto \left(\begin{array}{llll}
a_{0,0} & 0 & a_{0,1} & a_{0,1} \\
0 & a_{0,0} & a_{0,1} & a_{0,1} \\
0 & 0 & a_{1,1} & 0\\
0 & 0 & 0 & a_{1,1}
\end{array}\right) $$
which is clearly not a ring homomorphism.
\begin{remark}\label{remark:fcc property}
Let $\Lambda^1$ be a proset and let $\sqcup_{i\in I}\Lambda_i$ the decomposition of $\Lambda^1$ into its components. Notice that if $f:\Lambda^1\rightarrow \Lambda^2$ is FCC then for every $s\in \Lambda^2$,\ $i\in I$ we have that either $f^{-1}(s)\cap \Lambda_i=\emptyset$, $f^{-1}(s)\cap \Lambda_i=\{t_i\}$ or $f^{-1}(s)\cap \Lambda_i=\Lambda_i$.
\end{remark}

%Notice that if $f:\Lambda_1\rightarrow \Lambda_2$ is a convex embedding,\ then the pre-image of convex subsets of $\Lambda_2$ is a convex subset of $\Lambda_1$.\\ \indent
\begin{defi}
We define the category category of locally finite prosets $\textbf{\textup{prosets}}_{\textup{fin}}$ as:
\begin{itemize}
    \item Objects: all locally finite prosets,
    \item Arrows: all the FCC morphisms between locally finite prosets.
\end{itemize}
\end{defi}

Notice that the category $\textbf{\textup{prosets}}_{\textup{fin}}$ has $0=\emptyset$ as its initial object and $1$ as its terminal object.\\
\indent Our goal now is to show that if $f$ is FCC then $\textbf{M}[f]$ can be extended to a ring homomorphism. Not only that,\ we can define a contravariant functor from the category $\textbf{prosets}_\text{fin}$ to $\textbf{TopRings}$.

\begin{theorem}\label{thrm:functor construction} \index{$\textbf{\textup{M}}_{\_}(P)$|ndx}\index{contravariant functor|ndx}
Let $P$ be a topological ring. The map 
$$\begin{array}{cccc}
 \textbf{\textup{M}}_{\_}(P):    & \textbf{\textup{prosets}}_{\textup{fin}}&\Longrightarrow & \textbf{\textup{TopRings}} \\
& \Lambda &\longmapsto     & \textup{M}_{\Lambda}(P)\\
& f& \longmapsto &\textbf{\textup{M}}[f]
\end{array}$$
is a contravariant functor.
\end{theorem}

\begin{proof}
Given $P$ a topological ring,\ the functor $\mathbf{M}_{\_}(P)$ maps the object $\Lambda$ from $posets$ to $\mathbf{M}_{\_}(P)(\Lambda):=\textup{M}_{\Lambda}(P)$,\ where $\textup{M}_\emptyset(P):=\{0\}$ is defined to be the trivial ring. We now need to show the functor map FCC maps to continuous ring homomorphims. To simplify the notation we will denote $\mathbf{M}_{\_}(P)(f):=\mathbf{M}[f]$,\ for $f$ an FCC map. The proof will follow by defining a map from the generators of the domain and showing it extends to a continuous ring homomorphism. Remark \ref{remark:relations among generators} and Proposition \ref{prop:dense subset rings} will be central for this part of the proof. It will then remain to show that composition of functions is mapped to composition of functions.\\
\indent If $\Lambda_1$ is the empty poset and $f:\emptyset\rightarrow \Lambda_2$ is the unique morphism from the empty set to $\Lambda_2$,\ define $\mathbf{M}[f]$ as the unique morphism from $\textup{M}_{\Lambda_2}(P)$ to $\textup{M}_\emptyset(P)$.\\
\indent For $\Lambda_2$ a non-empty set,\ we extend $\mathbf{M}[f]$ for some finite sums as follows:
\begin{itemize}
    \item If $A,B\in \{p^{\Lambda}\}_{p\in P}\cup \{e^{(s_1,s_2)}\}_{s_1  \preceq s_2\in\Lambda_2}$,\ the generating set,\ we define $$\mathbf{M}[f](A+B):=\mathbf{M}[f](A)+\mathbf{M}[f](B).$$
    \item If $A\in \{e^{(s_1,s_2)}\}_{s_1  \preceq s_2\in\Lambda_2}$ and $p\in P$,\ we define 
    $$p^{\Lambda_1}\mathbf{M}[f](A)=\mathbf{M}[f](p^{\Lambda_2}A)=\mathbf{M}[f](Ap^{\Lambda_2})=\mathbf{M}[f](A)p^{\Lambda_1}.$$
\end{itemize}

We want now to show that such a map can be extended to a continuous ring homomorphism. First,\ we will show that such a map can be extended to a ring homomorphism on the dense subset from Proposition \ref{prop:dense subset rings} and then extend it continuously to the whole ring. For that let $\Lambda_1=\sqcup_{i\in I}\Lambda_i$ the decomposition of $\Lambda_1$ into its irreducible components.

\indent \textit{Claim 1}: Let $t_1\precnapprox t_2\in \Lambda_1$ be such that $f(t_1)=s_1$ and $f(t_2)=s_2$ for some $s_1\precnapprox s_2\in\Lambda_2$. If $s_1\precnapprox s_2\precnapprox s_3$,\ for some $s_3\in \Lambda_2$ then one of the following happen:
\begin{itemize}
    \item $e^{(t_1,t_2)}\mathbf{M}[f](e^{(s_2,s_3)})=0$,\ or
    \item $e^{(t_1,t_2)}\mathbf{M}[f](e^{(s_2,s_3)})=e^{(t_1,t_3)}$ for a unique $t_3\in\Lambda_1$ such that $t_1\precnapprox t_2\precnapprox t_3$ and $f(t_3)=s_3$.
\end{itemize}
Assume $e^{(t_1,t_2)}\mathbf{M}[f](e^{(s_2,s_3)})\neq 0$. Then expanding it,\ we have the right-hand side of
$$e^{(t_1,t_2)}\mathbf{M}[f](e^{(s_2,s_3)})=e^{(t_1,t_2)}\left(\sum e^{(t_2',t_3')} \right)$$
has at least one pair $(t_2',\ t_3')$ such that $f(t_2')=s_2$,\ $t_2'=t_2$,\ and $f(t_3')=s_3$ (Remark \ref{remark:relations among generators}). Hence, restricted to the component containing $t_1,\ t_2$ the function $f$ is a convex embedding. By Remark \ref{remark:fcc property},\ such the pair $(t_2',\ t_3')$ is unique, as it has to be on the same component as $t_1,\ t_2$. That is,\ if $e^{(t_1,t_2)}\mathbf{M}[f](e^{(s_2,s_3)})\neq 0$ then $e^{(t_1,t_2)}\mathbf{M}[f](e^{(s_2,s_3)})=e^{(t_1,t_3')}$.\\
\indent \textit{Claim 2}: Let $s_1\precnapprox s_2$ be elements in $\Lambda_2$. Then $\mathbf{M}[f](e^{(s_1,s_2)})\mathbf{M}[f](e^{(t_1,t_2)})=\mathbf{M}[f](e^{(s_1,s_2)}e^{(t_1,t_2)})$ for every $t_1,\ t_2\in \Lambda_2$.\\
\indent Assume $s_1,\ s_2,\ t_1,\ t_2\in\Lambda_2$ are such that $s_1\precnapprox s_2$,\ $s_2=t_1$ and $t_1\precnapprox t_2$,\ as otherwise the result would be trivially $0$ on both sides. Then $e^{(s_1,s_2)}e^{(t_1,t_2)}=e^{(s_1,t_2)}$ and,\ as $f$ is FCC,\ by Remark \ref{remark:fcc property} the right-hand side is
\begin{equation}\label{equation:left_hand}
\mathbf{M}[f](e^{(s_1,t_2)})=\sum_{j\in J}e^{(q_{j_1},q_{j_2})}    
\end{equation}
for $J$ a subset of $I$,\ $q_{j_1}\precnapprox q_{j_2}\in\Lambda_j$ and $f^{-1}(s_1)\cap \Lambda_j=\{q_{j_1}\}$,\ $f^{-1}(t_2)\cap \Lambda_j=\{q_{j_2}\}$. For the left-hand side,\ 
\begin{equation}\label{equation:right_hand}
\mathbf{M}[f](e^{(s_1,s_2)})\mathbf{M}[f](e^{(t_1,t_2)})=\left(\sum_{k\in K}e^{(s_{k_1},s_{k_2})}\right)\left(\sum_{l\in L}e^{(t_{l_1},t_{l_2})}\right)    
\end{equation}
where $K$ and $L$ are subsets of $I$,\ for $k\in K$ we have $s_{k_1}\precnapprox s_{k_2}\in\Lambda_k$,\ $f^{-1}(s_1)\cap \Lambda_k=\{s_{k_1}\}$,\ $f^{-1}(s_2)\cap \Lambda_k=\{s_{k_2}\}$ and for $l\in L$ we have $t_{l_1}\precnapprox t_{l_2}\in\Lambda_l$,\ $f^{-1}(t_1)\cap \Lambda_l=\{t_{l_1}\}$,\ $f^{-1}(t_2)\cap \Lambda_l=\{t_{l_2}\}$. As we assumed $s_1\precnapprox s_2=t_1\precnapprox t_2$ we have that
$$\mathbf{M}[f](e^{(s_1,s_2)})\mathbf{M}[f](e^{(t_1,t_2)})=\left(\sum_{p\in K\cap L}e^{(s_{p_1},t_{p_2})}\right).$$
We need to show $K\cap L=J$,\ and the result will follow from Remark \ref{remark:fcc property}. If $j\in J$ then there are $q_{j_1}\precnapprox q_{j_2}$ such that $f(q_{j_1})=s_1$,\ $f(q_{j_2})=t_2$,\ hence $f|_{\Lambda_j}$ is convex embedding. Then there is $q\in[q_{j_1},q_{j_2}]$ such that $f(q)=s_2=t_1$,\ that is,\ $e^{(q_{j_1},q)}$ and $e^{(q,q_{j_2})}$ show up as terms in the right hand side of \ref{equation:right_hand}. Hence $j\in K\cap L$.\\
\indent On the other hand,\ if $p\in K\cap L$,\ then there are $s_{p_1}\precnapprox t\precnapprox t_{p_2}\in \Lambda_p$ such that $f(s_{p_1})=s_1$,\ $f(t)=s_2=t_1$,\ $f(t_{p_2})=t_2$. Hence the term $e^{(s_1,t_2)}$ appears on the right-hand side of Equation \ref{equation:left_hand}. That is,\ $p\in J$.\\
%,\ where $L,\ K\subset I$,\ $t_{l_1}\precnapprox t_{l_2}\in \Lambda_l$ ,$f(t'_1)=t_1$,\ $f(t'_2)=t_2$,\ $s'_1\precnapprox s'_2$,\ $f(s'_1)=s_1$,\ $f(s'_2)=s_2$. By Remark \ref{remark:relations among generators} ,\ when expanding the right-hand side of (\ref{equation:right_hand}) 
%\begin{equation}\label{eq:extra_eq}
%\mathbf{M}[f](e^{(s_1,s_2)})\mathbf{M}[f](e^{(t_1,t_2)})=\sum_{q'_1,q'_2}e^{(q'_1,q'_2)}
%\end{equation}
%,\ for $q'_1,q'_2\in\Lambda_1$ such that $f(q'_1)=s_1$,\ $f(q'_2)=t_2$. As $f$ is FCC,\ if $e^{(q_1,q_2)}$ shows up on (\ref{equation:left_hand}) then there exists $q\in [q_1,q_2]$ such that $f(q)=s_2=t_1$. Hence $e^{(q_1,q)},\ e^{(q,q_2)}$ shows up on the right-hand side of (\ref{equation:right_hand}). Hence $e^{(q_1,q_2)}$ is a term (\ref{eq:extra_eq}).\\
%\indent In a similar way,\ if $e^{(q_1',q_2')}$ is a term of the right-hand side of (\ref{eq:extra_eq}) then there exists $q\in [q_1',q_2']$ such that $e^{(q_1',q')},\ e^{(q',q_2')}$
%are on the right-hand side of (\ref{equation:right_hand}),\ hence $q_1'\precnapprox q\precnapprox q_2'$,\ $f(q_1')=s_1$,\ $f(q')=s_2=t_1$,\ $f(q_2')=t_2$. That is,\ the term $e^{(q_1',q_2')}$ is a term of the right-hand side of (\ref{equation:left_hand}). Hence,\ the right-hand side of (\ref{equation:left_hand}) is equal to the right-hand side of (\ref{equation:right_hand}),\ proving the claim.\\
%With a similar argument to Claim 1. we have that for each $q_1'\in f^{-1}(s_1)$ there exists a unique $q_2'\in f^{-1}(s_2)$ such that $e^{(q_1',q_2')}$ shows up in the sum above. then implies that $\sum_{q'_1,q'_2}e^{(q'_1,q'_2)}$ is equal to the right-hand side of (\ref{equation:left_hand}). \\
\indent \textit{Claim 3}: $\mathbf{M}[f]$ is well-defined and continuous.\\
\indent Claim $1.$ and $2.$ implies it is well-defined for all elements that are finite sums and finite products of the generators. Hence it is well-defined for a dense subset of $\textup{M}_{\Lambda_2}(P)$ (Corollary \ref{prop:dense subset rings}). Given $\{A_\alpha\}_{\alpha\in \Gamma(\Lambda_2)}\subset \langle \{p^{\Lambda_2}\}_{p\in S},\ \{e^{(s_1,s_2)}\}_{s_1  \preceq s_2\in\Lambda_2} \rangle $ a convergent net,\ Corollary \ref{coro:nets in these rings} then implies
$$\mathbf{M}[f]\left(\lim_{\alpha\in \Gamma(\Lambda_2)}(A_\alpha)\right)=\lim_{\alpha\in \Gamma(\Lambda_2)}\mathbf{M}[f](A_\alpha).$$
Hence the morphism can be extended to a continuous ring homomorphism.\\
\indent \textit{Claim 4}: Given $f_1:\Lambda_1\rightarrow \Lambda_2$ and $f_2:\Lambda_2\rightarrow\Lambda_3$ then $\mathbf{M}[f_2\circ f_1]=\mathbf{M}[f_1]\circ\mathbf{M}[f_2]$.\\
\indent The result is trivial when $\Lambda_1=\emptyset$. Assume $\Lambda_1\neq \emptyset$. The proof will be given by looking at where the generators of $\textup{M}_{\Lambda_3}$ are mapped.\\
\indent It is easy to see that for $p\in P$
$$\textbf{M}[f_2\circ f_1](p^{(\Lambda_3})=p^{\Lambda_1}=\textbf{M}[f_1]\circ \textbf{M}[f_2](p^{\Lambda_3}).$$
\indent For the $e^{(s_1,s_2)}$ case,\ notice that if $\mathbf{M}[f_2\circ f_1](e^{(s_1,s_2)})\neq 0$ then:\\
\begin{equation}\label{eq:3}
    \begin{array}{lll}
    \mathbf{M}[f_2\circ f_1](e^{(s_1,s_2)})& = \sum_{t_1,t_2}e^{(t_1,t_2)}    &  \mbox{for }t_1\preceq t_2\in\Lambda_1,\ \mbox{and }f_2\circ f_1(t_1)=s_1,\\
    &  &  f_2\circ f_1(t_2)=s_2
\end{array}
\end{equation}
and 
\begin{equation}\label{eq:4}
\begin{array}{lll}
  \mathbf{M}[f_1]\circ\mathbf{M}[f_2](e^{(s_1,s_2)})&  =\mathbf{M}[f_1](\sum_{q_1,q_2}e^{(q_1,q_2)})    &  \mbox{where }q_1\preceq q_2\in\Lambda_2 \mbox{ and }f_2(q_1)=s_1,\ \\
    & &    f_2(q_2)=s_2\\
  &   = \sum_{q_1,q_2}(\sum_{t_1,t_2}e^{(t_1,t_2)})&\mbox{for }t_1\preceq t_2 \in \Lambda_1,\ \mbox{ and }f_2(q_1)=s_1,\ \\
  & &   f_2(q_2)=s_2,\ f_1(t_1)=q_1,\ f_1(t_2)=q_2.
\end{array}    
\end{equation}
Claim 1 implies that the right-hand side of Equation (\ref{eq:4}) has to be the same as the right-hand side of Equation (\ref{eq:3}). Then $\mathbf{M}[f_1]\circ\mathbf{M}[f_2](e^{(s_1,s_2)})=\mathbf{M}[f_2\circ f_1](e^{(s_1,s_2)})$.\\
\indent It then follows that $\mathbf{M}_{\_}(P)$ is a contravariant functor.

\end{proof}

We call the functor $\mathbf{M}_{\_}(P)$ the \textbf{incidence functor}\index{incidence funtor|ndx}.

\begin{remark}\label{remark:surj mapped to inj}
Notice that given $f:\Lambda^1\rightarrow \Lambda^2$ an FCC map and two elements $e^{(s_1,s_2)},\ e^{(t_1,t_2)}$ on the generator set of $M_{\Lambda^2}(P)$, if they are distinct and have no trivial image then the image under $\mathbf{M}[f]$ of both elements are disjoint. Hence if $f$ is a surjective FCC map we have that $\mathbf{M}[f]$ is injective.
\end{remark}

%Now that we have the functor,\ it is interesting to also understand why the categories were defined in the way they were. We now will make some comments on why the conditions of $f$ is FCC is necessary for the functions $\mathbf{M}[f]$ as defined in Theorem \ref{thrm:functor construction} be well-defined.




\subsection{Sending colimits to limits} 

In this section we will work with properties of the category $posets$ that later can be used to show our contravariant functor maps colimits to limits.

\begin{lemma}\label{lemma:existence coproducts posets}\index{$\textbf{\textup{prosets}}_{\textup{fin}}$|ndx}
Given $\{\Lambda_i\}_{i\in I}$ be an arbitrary collection of objects in $\textbf{\textup{prosets}}_{\textup{fin}}$,\ their coproduct exist and it is $\sqcup_{i\in I}\Lambda_i$,\ as defined in Definition \ref{defi:disjoint union prosets}.
\end{lemma}

\begin{proof}
Let $\{\Lambda_i\}_{i\in I}$  as in the statement and define $\Lambda:=\sqcup_{i\in I}\Lambda_i$. For each $i\in I$ let $i_i:\Lambda_i\rightarrow\Lambda$ be the embeddings sending $\Lambda_i$ to its copy in $\Lambda$.\\
\indent Claim: $\Lambda$ is the coproduct of  $\{\Lambda_i\}_{i\in I}$.\\
\indent Let $\Lambda'$ be another locally finite proset and,\ for each $i\in I$,\ let $f_i:\Lambda_i\rightarrow \Lambda'$ a FCC map. Define $(f_i)_{i\in I}:\Lambda\rightarrow \Lambda'$ by $(f_i)_{i\in I}(s_i)=f_i(s_i)$ if $s_i\in \Lambda_i$. It is clear that $(f_i)_{i\in I}\circ i_i=f_i$ and $(f_i)_{i\in I}$ is the unique FCC morphism satisfying this property. Hence $\Lambda$ is the coproduct of the collection $\{\Lambda_i\}_{i\in I}$.

$$% https://tikzcd.yichuanshen.de/#N4Igdg9gJgpgziAXAbVABwnAlgFyxMJZABgBoAmAXVJADcBDAGwFcYkQAdDgGXoFsARlHoB9LCAC+pdJlz5CKMsWp0mrdl16Dhk6SAzY8BIuQoqGLNok49+Q+gHJJKmFADm8IqABmAJwh8SACMNDgQSKYgjPQCMIwACrJGCiBYYNiwIDQW6tbeWVFpViDCcAAWrro+-oGIZCBhwTTRsQlJ8uxpGWzZasVYYlUgfgFI9Y2IkS1xiYYd1l1Ymb2W7N6DEpQSQA
\begin{tikzcd}
\Lambda \arrow[rrdd, "(f_i)_{i\in I}" description, dashed]                         &  &          \\
                                                                      &  &          \\
\Lambda_i \arrow[uu, "i_i" description] \arrow[rr, "f_i" description] &  & \Lambda'
\end{tikzcd}$$
\end{proof}

The following follows directly from Lemma \ref{lemma:existence coproducts posets} and Proposition \ref{prop:disjoint union and product rings}.

\begin{coro}\label{coro:functor maps coproducts to products}
The incidence functor $\mathbf{M}_\_(P)$ maps coproducts to products.
\end{coro}

\begin{defi}[Quotient order]
Let $\Lambda=\sqcup_{i\in I}\Lambda_i$ be a poset with order given by the disjoint union. We will say $\equiv\subset \Lambda\times\Lambda$ is a \textbf{FCC equivalence relation} if there is a FCC surjective map $f:\Lambda\rightarrow \Lambda'$ such that given $s_1,s_2\in \Lambda$ then $s_1\equiv s_2$ if,\ and only if,\ $f(s_1)=f(s_2)$. We write $\Lambda':=\Lambda/\equiv$ and call this set the \textbf{FCC quotient} under $\equiv$.
%given $s_1\sim s_2$ then or $s_1=s_2$,\ or if $s_1\neq s_2$ and exists $i\in I$ such that $s_1,s_2\in \Lambda_i$ then for every $s\in \Lambda_i$ we have $s\sim s_1$,\ or there exists $i_1\neq i_2\in I$ such that $s_1\in \Lambda_{i_1}$ and $s_2\in \Lambda_{i_2}$. The \textbf{quotient} will be denoted $\Lambda/\sim$ with elements the equivalence classes under this relation. For $[t_1],[t_2]\in \Lambda/\sim$,\ we define the quotient order as $[t_1]\leqslant [t_2]$ if there exists $q_1\in [t_1]$,\ $q_2\in [t_2]$ and $s_1,s_2\in \Lambda$ such that $q_1\leqslant s_1\sim s_2 \leqslant q_2$.
\end{defi}

For the next result we will prove the existence of pushouts in the category $\textbf{\textup{prosets}}_{\textup{fin}}$. We will first give a remark on how such construction works in the case the proset $\Lambda$ is irreducible,\ and the proof will then be given for the general case.

\begin{remark}
Let $\Lambda$,\ $\Lambda_1$ and $\Lambda_2$ be prosets and $f:\Lambda\rightarrow \Lambda_1$,\ $g:\Lambda\rightarrow \Lambda_2$ be FCC maps. We want to build the pushout diagram:
$$% https://tikzcd.yichuanshen.de/#N4Igdg9gJgpgziAXAbVABwnAlgFyxMJZABgBpiBdUkANwEMAbAVxiRAB12AZOgWwCModEAF9S6TLnyEUZAIxVajFm048BQgPoAmUeJAZseAkTnlF9Zq0QdufQXU1y9Eo9NOkF1Syptr7WsAAZqQA5iKiijBQofBEoEEAThC8SGQgOBBIZiAMdPwwDAAKksYyIFhg2LAg3srWIKEuIEkpadSZSNrUeQXFpe42ldWsdVZsQc2tqYjdGVmIAMw9+YUlbiZDVVg1Y74GTlPJMzmdS3sNaDq1uav9G+XDO6wiFCJAA
\begin{tikzcd}
\Lambda \arrow[d, "g" description] \arrow[r, "f" description] & \Lambda_1 \arrow[d, "p_1" description] \\
\Lambda_2 \arrow[r, "p_2" description]                        & {\Lambda_{f,g}}                       
\end{tikzcd}$$
For the case $\Lambda=\emptyset$,\ as the empty set is the initial object of $\textbf{\textup{prosets}}_{\textup{fin}}$,\  $\Lambda_{f,g}=\Lambda_1\sqcup \Lambda_2$ and $p_1$,\ $p_2$ are the embeddings of $\Lambda_1,\ \Lambda_2$ into $\Lambda_1\sqcup \Lambda_2$.\\
\indent Assume $\Lambda$ is irreducible and non-empty. As $\Lambda$ is irreducible,\ there exists an unique $j_0\in J$ and $k_0\in K$ such that $f(\Lambda)\subset \Lambda_j$,\ $g(\Lambda)\subset \Lambda_k$. The desired proset $\Lambda_{f,g}$ will be as follows: 
$$\Lambda_{f,g}=\left(\bigsqcup_{j\in J\backslash\{j_0\}}\Lambda_j \right)\sqcup\left(\bigsqcup_{k\in K\backslash\{k_0\}}\Lambda_k \right)\sqcup \Lambda_{\{j_0,k_0\}}.$$
The proset $\Lambda_{\{j_0,k_0\}}$ is the FCC quootient $\Lambda_{j_0}\sqcup \Lambda_{k_0}$ with equivalence relation given by:
\begin{itemize}
    \item for every $t\in \Lambda$,\ $f(t)\equiv g(t)$,
    \item if $\Lambda\neq 1$,\ $f$ is a convex embedding and $g$ is a constant function then for every $s_1,\ s_2\in \Lambda_{j_0}$ we have $s_1\equiv s_2$,
    \item if $\Lambda\neq 1$,\ $g$ is a convex embedding and $f$ is a constant function then for every $s_1,\ s_2\in \Lambda_{k_0}$ we have $s_1\equiv s_2$.
\end{itemize}
This is the maximal FCC quotient of $\Lambda_{j_0}\sqcup \Lambda_{k_0}$ such that $\pi\circ i_{j_0}\circ f= \pi \circ i_{k_0}\circ g$. Here the maps
$\pi:\Lambda_{j_0}\sqcup \Lambda_{k_0}\rightarrow \Lambda_{\{j_0,k_0\}}$ is given by the FCC quotient under $\equiv$,\ and $i_{j_0}$,\ $i_{k_0}$ are the embeddings from $\Lambda_{j_0}$,\ $\Lambda_{k_0}$ into their respective components in the disjoint union $\Lambda_{j_0}\sqcup\Lambda_{k_0}$. It is then the case 
\begin{itemize}
    \item $p_1|_{\Lambda_{j_0}}=\pi\circ i_{j_0}$,
    \item for $j\neq j_0$,\ $p_1|_{\Lambda_j}=i_j$,
    \item $p_2|_{\Lambda_{k_0}}=\pi \circ i_{k_0}$,
    \item and for $k\neq k_0$,\ $p_2|_{\Lambda_k}=i_k$.
\end{itemize}
As $p_1$,\ $p_2$ is defined on all the components of $\Lambda_{\{f,g\}}$,\ it is uniquely defined for the whole proset. Notice that $\Lambda_{f,g}$ is an FCC quotient of $\Lambda_1\sqcup \Lambda_2$.
\end{remark}

\begin{lemma}\label{lemma:existence of pushouts}
Let $\Lambda,\Lambda_1,\Lambda_2$ be locally finite prosets and $f:\Lambda\rightarrow \Lambda_1$,\ $g:\Lambda\rightarrow \Lambda_2$ FCC maps. Then there exists $\Lambda_{f,g}$ a locally finite proset and $p_1:\Lambda_1\rightarrow \Lambda_{f,g}$,\ $p_2:\Lambda_2\rightarrow \Lambda_{f,g}$ FCC maps such that the diagram
$$% https://tikzcd.yichuanshen.de/#N4Igdg9gJgpgziAXAbVABwnAlgFyxMJZABgBpiBdUkANwEMAbAVxiRAB12AZOgWwCModEAF9S6TLnyEUZAIxVajFm048BQgPoAmUeJAZseAkTnlF9Zq0QdufQXU1y9Eo9NOkF1Syptr7WsAAZqQA5iKiijBQofBEoEEAThC8SGQgOBBIZiAMdPwwDAAKksYyIFhg2LAg3srWIKEuIEkpadSZSNrUeQXFpe42ldWsdVZsQc2tqYjdGVmIAMw9+YUlbiZDVVg1Y74GTlPJMzmdS3sNaDq1uav9G+XDO6wiFCJAA
\begin{tikzcd}
\Lambda \arrow[d, "g" description] \arrow[r, "f" description] & \Lambda_1 \arrow[d, "p_1" description] \\
\Lambda_2 \arrow[r, "p_2" description]                        & {\Lambda_{f,g}}                       
\end{tikzcd}$$
is a pushout diagram.
\end{lemma}

\begin{proof}
For the proof we will write $\Lambda=\sqcup_{i\in I}\Lambda_i$,\ $\Lambda_1=\sqcup_{j\in J}\Lambda_j$ and $\Lambda_2=\sqcup_{k\in K}\Lambda_k$ the decomposition of these sets into their components.\\
\indent
%For each $i\in I$ define $f_i:=f|_{\Lambda_i}$,\ $g_i:=g|_{\Lambda_i}$,\ $j_i\in J$ the element such that $f_i(\Lambda_i)\subset \Lambda_{j_i}$ and $k_i\in K$ the element such that $g_i(\Lambda_i)\subset \Lambda_{k_i}$. 
Define the sets:
$$\begin{array}{l}
    J_0=\{j\in J:\  \text{for all }i\in I,\ f(\Lambda_i)\cap \Lambda_j=\emptyset\}\subset J\\
    J_1=\{j\in J\backslash J_0:\  \forall i\in I,\ \text{ if }f(\Lambda_i)\subset \Lambda_j \text{ then }f|_{\Lambda_i} \text{ is a convex embedding}\}\subset J \\ 
    J_2=\{j\in J\backslash J_0:\  \forall i\in I,\ \text{ if }\Lambda_i\neq 1,\ f(\Lambda_i)\subset \Lambda_j \text{ then }f|_{\Lambda_i} \text{ is a constant function}\}\subset J \\ 
    J_3=J\backslash (J_0\cup J_1\cup J_2) \\
    K_0=\{k\in K:\  \text{for all }i\in I,\ g(\Lambda_i)\cap \Lambda_k=\emptyset\}\subset K\\
    K_1=\{k\in K\backslash K_0:\  \forall i\in I,\ \text{ if }g(\Lambda_i)\subset \Lambda_k \text{ then }g|_{\Lambda_i} \text{ is a convex embedding}\}\subset K  \\
    K_2=\{k\in K\backslash K_0:\  \forall i\in I,\ \text{ if }\Lambda_i\neq 1,\ g(\Lambda_i)\subset \Lambda_k \text{ then }g|_{\Lambda_i} \text{ is a constant function}\}\subset K  \\
    K_3= K\backslash (K_0\cup K_1 \cup K_2).
\end{array}$$
For each $l\in J\sqcup L$ also define the set $\langle l\rangle$ as the minimal set such that:
\begin{itemize}
    \item $l\in \langle l\rangle$.
    \item Let $k\in K$ be such that $k\in \langle l\rangle$. If $i\in I$ is such that $g(\Lambda_i)\subset \Lambda_k$ and $f(\Lambda_i)\subset \Lambda_j$,\ then $j\in \langle l\rangle$. 
    \item Let $j\in J$ be such that $j\in \langle l\rangle$. If $i\in I$ is such $f(\Lambda_i)\subset \Lambda_j$ and $g(\Lambda_i)\subset \Lambda_k$,\ then $k\in \langle l\rangle$. 
\end{itemize}
In other words,\ $\langle l\rangle$ is the set of components that contains $\Lambda_l$ and that will be ``glued together'' under the pushout. Notice that if $l\in J_0\sqcup K_0$ then $\langle l\rangle=\{l\}$. \\
\indent Let $L=\{\langle l\rangle:\  l\in J\sqcup K\}$ the partition of $J\sqcup K$ defined as above. Define $\Lambda_{f,g}$ as follows:
$$\Lambda_{f,g}:=\bigsqcup_{\langle l\rangle\in L}\Lambda_{\langle l\rangle}$$
where $\Lambda_{\langle l\rangle}$ is defined as
$$\Lambda_{\langle l\rangle}=\left.\left(\bigsqcup_{l\in \langle l\rangle}\Lambda_l\right)\right/\equiv_{l}$$
where
\begin{itemize}
    \item for every $s\in \Lambda$,\ if there is $l\in \langle l\rangle$ such $f(s)\in \Lambda_l$ then $f(s)\equiv_{l} g(s)$.
    \item if $l\in \langle l\rangle$ is such that $l\in J_3\cup K_3$ then for every $s_1,\ s_2\in \Lambda_l$ we have $s_1\equiv_{l} s_2$.
    \item if $j\in J_1$ and $k\in K_2$ are such that there is $i\in I$ with $f(\Lambda_i)\subset \Lambda_j$,\ $g(\Lambda_i)\subset \Lambda_k$ then for every $s_1,\ s_2\in \Lambda_j$  we have $s_1\equiv_{l} s_2$.
    \item if $j\in J_2$ and $k\in K_1$ are such that there is $i\in I$ with $f(\Lambda_i)\subset \Lambda_j$,\ $g(\Lambda_i)\subset \Lambda_k$ then for every $s_1,\ s_2\in \Lambda_k$ we have $s_1\equiv_{l} s_2$.
\end{itemize}
with the order given by the FCC quotient. Notice that the construction is similar to the irreducible case,\ but here we have more components being ``glued together''. Notice that $\Lambda_{f,g}=(\Lambda_1\sqcup \Lambda_2)/\equiv$,\ for the $\equiv$ FCC equivalence relation defined above on each component $\Lambda_{\langle l\rangle}$. Let $i_1:\Lambda_1 \rightarrow\Lambda_1\sqcup \Lambda_2$ and $i_2:\Lambda_2\rightarrow \Lambda_1\sqcup \Lambda_2$ the embeddings from the coproduct and $\pi:\Lambda_1\sqcup \Lambda_2\rightarrow \Lambda_{f,g}$ given by the FCC quotient. We then define $p_1:=\pi\circ i_1$ and $p_2:=\pi\circ i_2$.\\
\indent Notice that $\Lambda_{f,g}$ is defined so that it is the maximal FCC quotient of $\Lambda_1\sqcup \Lambda_2$ such that there exists an unique FCC maps $p_1$,\ $p_2$ with $p_1\circ f=p_2\circ g$. The construction implies that if there are FCC maps $f':\Lambda_1\rightarrow \Lambda'$ and $g':\Lambda_2\rightarrow \Lambda'$,\ then there exists a unique FCC map $p':\Lambda_{f,g}\rightarrow \Lambda'$ such that $f'=p'\circ p_1$ and $g'=p'\circ p_2$. 
$$% https://tikzcd.yichuanshen.de/#N4Igdg9gJgpgziAXAbVABwnAlgFyxMJZABgBpiBdUkANwEMAbAVxiRAB12AZOgWwCModEAF9S6TLnyEUZAIxVajFm048BQgPoAmUeJAZseAkTnlF9Zq0QdufQXU1y9Eo9NOkF1Syptr7WsAAZqQA5iIuBpLGMsjapNoWyta26g4A5KKKMFCh8ESgQQBOELxIZCA4EEhmIAx0-DAMAArR7jZYYNiwIN7JbKGRxaXl1FVI8XUNTa1uJh1dWD19VmxBQyVliJPjiADM1PWNLW3zIJ3drCu+Bk4bI4i1uwdKqzZoOr1Tx7NSZxdLVhiQqbGpjaqIAAsh2mJzmMnOi2WrxuoUywJAwy2Owh0O+M1OCIByJ8KSC6P0WKQL12eKOBPhbGJVzqnRSQjgAAscl9SWw0FkREA
\begin{tikzcd}
\Lambda \arrow[d, "g" description] \arrow[r, "f" description]        & \Lambda_1 \arrow[d, "p_1" description] \arrow[rdd, "f'" description] &          \\
\Lambda_2 \arrow[r, "p_2" description] \arrow[rrd, "g'" description] & {\Lambda_{f,g}} \arrow[rd, "p'" description, dashed]                  &          \\
                                                                     &                                                                      & \Lambda'
\end{tikzcd}$$
\end{proof}

%The following isomorphism theorem for FCC maps follows trivially from definition.

%\begin{lemma}\label{lemma:image as quotient}
%Let $f:\Lambda_1\rightarrow\Lambda_2$ be an FCC embedding. Then $Im(f)\cong \Lambda_1/\sim$ for some FCC relation.
%\end{lemma}
Note that the intuitive idea of pushouts of prosets is getting two prosets,\ $\Lambda_1$ and $\Lambda_2$,\ with some common convex subsets,\ given by the maps $f$ and $g$ on each component of $\Lambda$,\ and making these subsets an intersection of them. Below we have an example of that:

\begin{ex}
Let $\alpha=\mathbf{2}<=\{0,1\}$,\ $\Lambda_1=\mathbf{Z}$ and $\Lambda_2=\mathbf{Zig}$ and define 
$$\begin{array}{llll}
    i_1: & \mathbf{2}< & \longrightarrow & \mathbf{Z}\\
     & 0 & \longmapsto & 0\\
    & 1 & \longmapsto & -1,
\end{array}
$$
and
$$\begin{array}{llll}
    i_2: & \mathbf{2}< & \longrightarrow & \mathbf{Zig}\\
     & 0 & \longmapsto & 0\\
    & 1 & \longmapsto & -1.
\end{array}$$
The pushout of this diagram is the following poset:
$$% 
\begin{tikzcd}
       &                          &                       &                                     &                      & \iddots \arrow[ld, dashed] &        \\
       &                          &                       &                                     & 1 \arrow[ld, dashed] &                           &        \\
       & -2 \arrow[rd] \arrow[ld] &                       & 0 \arrow[ld, Rightarrow] \arrow[rd] &                      & 2 \arrow[ld] \arrow[rd]   &        \\
\ldots &                          & -1 \arrow[ld, dashed] &                                     & 1                    &                           & \ldots \\
       & -2 \arrow[ld, dashed]    &                       &                                     &                      &                           &        \\
\iddots &                          &                       &                                     &                      &                           &       
\end{tikzcd}$$
Where the normal arrow represents the element of $\mathbf{Zig}$,\ the dashed arrows are the elements from $\mathbf{Z}$ and the double arrow represent the elements ``glued together'' under the pushout.
\end{ex}

Notice that as $\emptyset$ is an initial object of $\textbf{\textup{prosets}}_{\textup{fin}}$ then this category has coequalizers (Proposition \ref{prop:coeq iff coprod}). We then get the following:

\begin{coro}
The category $\textbf{\textup{prosets}}_{\textup{fin}}$ has all colimits.
\end{coro}

\begin{proof}
By Lemmas \ref{lemma:existence coproducts posets} and \ref{lemma:existence of pushouts} and Proposition \ref{prop:having_all_limits} our results follows.
\end{proof}

And as the category of $\textbf{\textup{prosets}}_{\textup{fin}}$ has only FCC maps and locally finite ordered sets,\ we get the following:

\begin{coro}
Colimits of FCC maps are FCC maps and they preserve the property of being locally finite.
\end{coro}

In other words,\ direct limits,\ pushouts and disjoint unions of locally posets under FCC maps are locally finite posets. We now will use these results to show that coequalizers are mapped to equalizers via $\mathbf{M}_{\_}(P)$.

\begin{remark}
Let $f,\ g:\Lambda^1\rightarrow \Lambda^2$ be two maps. Let $\{\Lambda_i\}_{i\in I}$ the set of components of $\Lambda^1$ and $\{\Lambda_j\}_{j\in J}$ the set of components of $\Lambda^2$. We define $\textup{Coeq}(f,\ g):=\Lambda^2/\equiv_{\textup{Coeq}}$ as follows:
\begin{enumerate}
    \item For all $t\in \Lambda^1$, $f(t)\equiv_{\textup{Coeq}}g(t)$.
    \item If $j\in J$ is such that there is $i\in I$, $t\in \Lambda_i$ with $f(t),\ g(t)\in \Lambda_j$ and $f(t)\neq g(t)$, then for every $s_1,\ s_2\in \Lambda_j$, $s_1\equiv_{\textup{Coeq}}s_2$.
\end{enumerate}
and the map $p:\Lambda^2\rightarrow \textup{Coeq}(f,\ g)$ as the quotient map. Notice that the first condition makes $p\circ f=p \circ g$, and the second condition is a minimal condition for the map $p$ to be FCC.
\end{remark}

\begin{lemma}\label{lemma:functor maps coequalizers to equalizers}
Let $f_1,\ f_2:\Lambda^1\rightarrow \Lambda^2$ and $p:\Lambda^2\rightarrow \textup{Coeq}(f_1,\ f_2)$ be the coequalizer of $f_1$ and $f_2$. Then $\mathbf{M}[p]$ is the equalizer of $\mathbf{M}[f_1],\ \mathbf{M}[f_2]$. 
\end{lemma}

\begin{proof}
First,\ let $f_1,f_2,\ p$ as in the statement. We first show that $\mathbf{M}[f_1]\circ\mathbf{M}[p]=\mathbf{M}[f_2]\circ\mathbf{M}[p]$. We then prove $\mathbf{M}[p]$ is the equalizer of $\mathbf{M}[f_1],\mathbf{M}[f_2]$.\\
\indent Notice that for $n=1,\ 2$:
$$\begin{array}{llll}
    \mathbf{M}[f_n]\circ\mathbf{M}[p]:& \textup{M}_{\textup{Coeq}(f_1,\ f_2)}(P) &\longrightarrow &  \textup{M}_{\Lambda^1}(P) \\
     & r^{\textup{Coeq}(f_1,\ f_2)} & \longmapsto & r^{\Lambda^1}\\
     & 1^{\{s\}} & \longmapsto & \left\{\begin{array}{ll}
                                            1^{(p\circ f_n)^{-1}(s)}   & \mbox{if }(p\circ f_n)^{-1}\neq\emptyset \\
                                            0     & \mbox{otherwise} 
     \end{array}\right. \\
     & e^{(s_1,s_2)}&\longmapsto & \left\{\begin{array}{ll}
                                          \sum_{t_1,t_2}e^{(t_1,t_2)}    &  \mbox{for }t_1\precnapprox t_2 \mbox{ and }p\circ f_n(t_1)=s_1,\ \\
                                           & p\circ f_n(t_2)=s_2\\
                                       0      &  \mbox{otherwise}
                                    \end{array}\right.    
\end{array}$$
Because $p$ is the coequalizer of $f_1$ and $f_2$ it follows that $\mathbf{M}[f_1]\circ\mathbf{M}[p]=\mathbf{M}[f_2]\circ\mathbf{M}[p]$. Notice that as $p$ is surjective,\ Remark \ref{remark:surj mapped to inj} implies $\mathbf{M}[p]$ is injective.\\
\indent Now let $\Lambda'$ be a poset and $h':{M}_{\Lambda'}(P)\rightarrow \textup{M}_{\Lambda^2}(P)$ be such that $\mathbf{M}[f_1]\circ h'=\mathbf{M}[f_2]\circ h'$ and $h'(r^{\Lambda'})=r^{\Lambda^2}$,\ for every $r\in P$. Define $h:\textup{M}_{\Lambda'}(P)\rightarrow \textup{M}_{\textup{Coeq}(f_1,\ f_2)}(P)$ as:
$$h(A)=\left\{\begin{array}{ll}
    (\mathbf{M}[p])^{-1}(h'(A)) & \mbox{if } (\mathbf{M}[p])^{-1}(h'(A))\neq\emptyset  \\
    0 & \mbox{otherwise.}
\end{array}\right.$$ 

\noindent This function is well-defined because $\mathbf{M}[p]$ is injective. Hence the following diagram commute:

$$% https://tikzcd.yichuanshen.de/#N4Igdg9gJgpgziAXAbVABwnAlgFyxMJZAFgBoAGAXVJADcBDAGwFcYkQBZAfWAB1eAMvQC2AIyj0uARgC+ACgAKAShAzS6TLnyEUAJgrU6TVu259BI8ZN3zlq9SAzY8BIuQM0GLNok49+QmISXADMtipqGs7abqS6hl4mvmYBlhIA5OGqhjBQAObwRKAAZgBOEMJIUjQ4EEjuIHAAFljFOEgAtCE0jPSiMIwKmi46IFhg2LAgnsY+IPzC9DhNosXAHDLIxZT2JeWViNUgtfU0za3thz19A0PRrr7jk2wz3uwLSytrG8h5O5EgMoVJDdY51RD6ECMcZzCTNXLTKE3QbDGKPCZYKavJIgJq7QH7EE1cFHXr9FH3UZPTEvIxvXxNdL4oEHSEnK5I8l3LQPMYYrF0nEfZardabND-SgyIA
\begin{tikzcd}
\textup{M}_{\textup{Coeq}(f_1,\ f_2)}(P) \arrow[rr, "{\mathbf{M}[p]}" description]                         &  & \textup{M}_{\Lambda^2}(P) \arrow[rr, "{\mathbf{M}[f_1]}" description, shift left=3] \arrow[rr, "{\mathbf{M}[f_2]}" description, shift right] &  & \textup{M}_{\Lambda^1}(P) \\
                                                                                   &  &                                                                                                                                 &  &                  \\
\textup{M}_{\Lambda'}(P) \arrow[uu, "h" description, dashed] \arrow[rruu, "h'" description] &  &                                                                                                                                 &  &                 
\end{tikzcd}$$
That is,\ $\mathbf{M}[p]$ is the equalizer of $\mathbf{M}[f_1],\ \mathbf{M}[f_2]$.
\end{proof} 

\begin{coro}\label{coro:functor maps colimits to limits}
The incidence functor $\mathbf{M}_{\_}$ sends colimits to limits.
\end{coro}

\begin{proof}
By Lemma \ref{lemma:functor maps coequalizers to equalizers} and Corollary \ref{coro:functor maps coproducts to products} we have that the functor $ ^{op}\circ\mathbf{M}_\_(P):\textbf{\textup{prosets}}_{\textup{fin}}\Rightarrow \textbf{TopRings}^{op}$ maps coequalizers to coequalizers and coproducts to coproducts. The result then follows from Proposition \ref{prop:sending_limits_to_limits}.
\end{proof}

\subsection{Generating the category \texorpdfstring{$\textbf{\textup{prosets}}_{\textup{fin}}$}{TEXT}}

In this section,\ we focus on showing that the prosets of the form $\mathbf{m}\leftarrow \mathbf{n}$,\ for $n,\ m\in\mathbb{N}$ can generate all locally finite prosets under direct limits,\ disjoint unions,\ and pushouts of FCC maps.\\
\indent The next result is the version of Theorem \ref{Prop: prodiscrete ring} in the category $\textbf{\textup{prosets}}_{\textup{fin}}$.

\begin{theorem}\label{thrm:direct limit posets finite intervals}
Let $\Lambda$ be an irreducible, locally finite proset. Then $\Lambda\cong\varinjlim_{\alpha\in\Gamma(\Lambda)}\alpha$,\ where $\Gamma(\Lambda)=\{\alpha\subset \Lambda: $ is finite and convex$\}$ with subset order.
\end{theorem}

\begin{proof}
For each $\alpha_1\subset\alpha_2\in \Gamma(\Lambda)$ let $j_{\alpha_2\rightarrow\alpha_1}:\alpha_1\rightarrow\alpha_2$ be the convex embedding given by the subset structure. It is clear that if $\alpha_1\subset\alpha_2\subset\alpha_3$ then $j_{\alpha_1\rightarrow\alpha_2}\circ j_{\alpha_2\rightarrow\alpha_3}=j_{\alpha_1\rightarrow\alpha_3}$,\ hence the direct limit $\varinjlim_{\alpha\in\Gamma(\Lambda)}\alpha$ exists. For each $\alpha_i\in\Gamma(\Lambda)$ let $i_{\alpha_i}:\alpha_i\rightarrow \Lambda$ be the embedding of $\alpha_i$ into $\Lambda$. Because the outer triangle of the following diagram commutes,\ there exists an unique $f:\varinjlim_{\alpha\in\Gamma(\Lambda)}\alpha\rightarrow \Lambda$ such that the whole diagram commutes.
$$% https://tikzcd.yichuanshen.de/#N4Igdg9gJgpgziAXAbVABwnAlgFyxMJZAJgBpiBdUkANwEMAbAVxiRAB136AnLMAKwZYAtgH1gnRmgAWdTn04BxOsOF0AFJwAyKgEZQ6ASgC+khjLohjpdJlz5CKAAykAzFVqMWbMxdHErGxAMbDwCIgAWNw96ZlZEDnYpWVEARkDbUIciMicYr3jEnWF9S2MPGCgAc3giUAAzbghhJBcQHAgkV2ohMEKDOGlKkB66XRgGAAU7MMcQPmxYEc84tnqMkEbmpDJ2zsRukAYxiems8ISFrCXqWO9L8V8U1OMNrZbEVOoOrtHxqZm2UuYEWrFuBTYWEeSXMKWIr2sDSaHy+e1af1OgIu8xB1zBK3uIH40OSdH8CKC7x2332bWO-zO9mxVxuBMKxIkML8LzeyOpaM+GIB5zmLPxd3ZJNhZOInF4VWkODo3CaAHcnmSeeVjEA
\begin{tikzcd}
                                                                                           &  & \Lambda                                                                         &  &                                                                                                                                                        \\
                                                                                           &  &                                                                                 &  &                                                                                                                                                        \\
                                                                                           &  & \varinjlim_{\alpha\in\Gamma(\Lambda)}\alpha \arrow[uu, "f" description, dashed] &  &                                                                                                                                                        \\
\alpha_2 \arrow[rruuu, "i_{\alpha_2}" description] \arrow[rru, "j_{\alpha_2}" description] &  &                                                                                 &  & \alpha_1 \arrow[lluuu, "i_{\alpha_1}" description] \arrow[llu, "j_{\alpha_1}" description] \arrow[llll, "j_{\alpha_2\rightarrow\alpha_1}" description]
\end{tikzcd}$$
By the direct limit property,\ $f$ is an FCC map and a direct limit of embeddings. Hence it is a convex embedding. To complete our proof,\ we will show that $f$ is surjective.\\
\indent Let $a\in \Lambda$. The set $\mathcal{N}_0(a)$ is a finite convex subset of $\Lambda$ containing $a$. It is clear that $f\circ j_{\mathcal{N}_0(a)}(a)=a$,\ hence $f$ is surjective.
\end{proof}


Lastly we can show a property which can be taken from the category $\textbf{prosets}_{\text{fin}}$ and translated to the context of matrix rings over $P$ indexed by a poset.

\begin{theorem}\label{thrm:creating prosets from countable class}
All objects in $\textbf{\textup{prosets}}_{\textup{fin}}$ are generated by $\mathbf{m}\leftarrow\mathbf{n}$,\ for $m,\ n\in\mathbb{N}$,\ and  under disjoint unions,\ direct limits and pushouts of convex embeddings.
\end{theorem}

\begin{proof}
We first prove by induction that we can generate all the irreducible,\ finite prosets. from The proof for this case will be by induction on the cardinality of $\Lambda$.\\
\indent Our generating set generates contains all irreducible posets of cardinalities $0$,\ $1$ and $2$,\ proving the base cases,\ as noted in Example \ref{ex:basic posets}. Assume the result is true for every irreducible $\Lambda$ with cardinality $k$,\ for some $k>2$.\\
\indent Let $\Lambda\notin\{\mathbf{i}\leftarrow\mathbf{j}\}_{i+j=k+1}$ be an irreducible proset with cardinality $k+1$. Let $a\neq b\in \Lambda$ such that  $\Lambda\backslash\mathcal{N}_0(a)$,\ $\Lambda\backslash\mathcal{N}_0(b)$, and $\Lambda\backslash(\mathcal{N}_0(a)\cup\mathcal{N}_0(b))$ are irreducible. Let $\alpha=\Lambda\backslash (\mathcal{N}_0(a)\cup\mathcal{N}_0(b))$,\ $\Lambda_1=\Lambda\backslash \mathcal{N}_0(a)$ and $\Lambda_2=\Lambda\backslash \mathcal{N}_0(b)$. Such elements $a,b$ exists as every finite connected graph with at least $3$ vertices has at least two non-cut vertices (a proof can be seen in \cite{graph-con-comp}). The conditions on $\Lambda$ imply $\Lambda\backslash(\mathcal{N}_0(a)\cup\mathcal{N}_0(b))$ is a non-empty set.\\
\indent Define $i_1:\alpha\rightarrow \Lambda_1$,\ $i_2:\alpha\rightarrow \Lambda_2$ the embeddings given by the subset structure. It follows that $|\Lambda_1|,|\Lambda_2|,|\alpha|<k+1$ and $\Lambda$ is the pushout of these prosets,\ proving our induction.\\
\indent Theorem \ref{thrm:direct limit posets finite intervals} implies that all infinite irreducible prosets are generated by finite,\ irreducible prosets under direct limits. Proposition \ref{defi:disjoint union prosets} implies that if all the irreducible posets are generated,\ so are the reducible ones under disjoint unions.
\end{proof} 

\begin{coro}\label{coro:building blocks for M_(P)}
The subclass of all rings of the form $\textup{M}_{\Lambda}(P)$,\ for $\Lambda$ a poset,\ is generated by $\textup{M}_{\mathbf{m}\leftarrow\mathbf{n}}(P)$,\ for $m,n\in\mathbb{N}$,\ under products,\ inverse limits and pullbacks.
\end{coro}

\begin{proof}
A direct corollary from Corollary \ref{coro:functor maps colimits to limits} and Theorem \ref{thrm:creating prosets from countable class}.
\end{proof}

This corollary can be useful for proving general properties of these rings. Instead of proving for all of them individually,\ you can prove for the generators and show that these properties are preserved by inverse limits and pullbacks.


%\begin{lemma}\cite[Lemma 2.1]{Matrices1985}
%    Let $\Lambda$ be a proset an $\{P_i\}_{i\in I}$ a collection of rings. Then $$\mathbf{M}_{\Lambda}(\prod_{i\in I}P_i)=\prod_{i\in I} \mathbf{M}_{\Lambda}(P_i)$$
%\end{lemma}

%\begin{coro}
%Let $P$ be a topological ring. The functor $^{op}\circ\mathbf{M}_{\_}(P):posets ^{op}\Rightarrow \textbf{TopRings}$ is left adjoint.
%\end{coro}

%\begin{proof}
%To prove this theorem we need to prove it satisfies the conditions from Theorem \ref{thrm:adjoint functor theorem}. \\
%\indent Define $\Lambda_{\aleph_0}:=\sqcup_{|\Lambda|<\aleph_0} \Lambda$,\ the disjoint union of all finite prosets. Given $R$ a topological ring,\ define $X_R$ the collection of all subsets of $\sqcup_{r\in R} \Lambda_{\aleph_0}$.\\
%\indent Now assume $f:R\rightarrow \textup{M}_{\Lambda}(P)$ is a ring homomorphism. There exists $\Lambda_f\subset \Lambda$ a locally convex collection of 
%\end{proof}

==> Sections/6-Comments.tex <==


\section{Other questions}\label{questions}

%\subsection{Isomorphism problem for matrix rings indexed by prosets}


%When working with the functor $\mathbf{M}_\_$ and with the isomorphism problem for rings of the form $\textup{M}_\Lambda(P)$ we focus on relations on the idempotents that only happen when $\Lambda$ is a poset. It might be possible to extend both results to prosets as well,\ but for that we need to find a way to manage the non-diagonal coordinate. A possible idea to solve such a problem is as follows:
%\begin{defi}\index{idempotent block|ndx}\index{dimension of the idempotent block|ndx}
%Let $\Lambda$ be a proset and $P$ a ring with only $\{0,\ 1\}$ as its sets of idempotents. Given $A\in \textup{M}_\Lambda(P)$ a minimal non-zero idempotent,\ define the set $[\![A]\!]$ as the minimal set satisfying:
%\begin{itemize}
 %   \item $A\in [\![A]\!]$.
  %  \item If $B\in [\![A]\!]$ and $C$ is a minimal non-zero element such that $CB=C$ and $BC=B$,\ then $5C\in[\![A]\!]$.
  %  \item If $B\in [\![A]\!]$ and $C$ is such that $C-B$ is topologically nilpotent,\ then $C\in [\![A]\!]$.
%\end{itemize}
%We call this set the idempotent block of $A$.\\
%\indent We define the dimension of $[\![A]\!]$ as:
%$$\dim ([\![A]\!])=\sup\{n:\ \exists A_1,\ldots,A_n\in [\![A]\!] \text{ such that }i\neq j \text{ implies }A_iA_j=0\}$$
%the cardinality of the maximal subset of perpendicular idempotents inside the block.
%\end{defi}
%For example,\ for the ring $\textup{M}_\mathbf{2}(\mathbb{Z})$,\ all the minimal non-zero idempotents are in the same block. It is also the case that for every $A\in \textup{M}_{\mathbf{2}}(\mathbb{Z})$ we have $\dim([\![A]\!])=2$. The goal would then show all the minimal non-zero idempotents of $\textup{M}_{\mathbf{n}}(P)$ are in the same block and that for every $A$ minimal non-zero idempotent of $\textup{M}_{\mathbf{n}}(P)$,\ $\dim([\![A]\!])=n$. The idea would then be using the blocks to find all blocks of square matrices in our ring and the relations from Lemma \ref{prop:isomorphism problem rings} to rebuild the proset structure from the matrix ring structure.

\subsection{Isomorphism problem for matrix groups}


When working with the isomorphism problem for $\textup{M}_\Lambda(P)$,\ we use relations between idempotents. As idempotents are not elements of the group,\ to prove the isomorphism problem for $\textup{GL}_\Lambda(P)$ it will be necessary to work with other properties of the groups and the ordered sets. It is already known a result that two non-isomorphic prosets can give isomorphic groups. To state such Theorem, given $\Lambda$ a proset, we define $\Lambda^{op}$ to be the proset with the same elements as $\Lambda$ and relation given by $x\preceq_{op} y$ in $\Lambda^{op}$ if, and only if, $y\preceq x$ in $\Lambda$. 
\begin{theorem}\cite[Theorem 1.21]{Matrices1973}
Let $\Lambda$ be a locally finite proset and $P$ a commutative ring. Then $\textup{GL}_{\Lambda}(P)\cong \textup{GL}_{\Lambda^{op}}(P)$.
\end{theorem}
For the case $\textup{aGL}_{\Lambda}(P)$,\ let $(\Lambda,\ \preceq_1)$ and $(\Lambda,\ \preceq_2)$ be prosets. If there are $S_1,\ldots,\ S_n$ finite subsets of $\Lambda$ such that $(\Lambda+\sum_{1\leqslant i \leqslant n}S_i,\ \preceq_{1+})$ is order isomorphic to $(\Lambda+\sum_{1\leqslant i \leqslant n}S_i,\ \preceq_{2+})$,\ then $\textup{aGL}_{\Lambda_1}(P)\cong \textup{aGL}_{\Lambda_2}(P)$. On the other hand,\ it is still not-known what are the general conditions for them to be isomorphic or not. In the article \cite{simple_matrices} it is given some conditions for these to be non-isomorphic when $\Lambda=\mathbb{Z}+\sum_{i\in I} \Lambda_i$,\ for some $\{\Lambda_i\}_{i\in I}$ locally convex collection of $\mathbb{Z}$.


\subsection{Alternative constructions}

The proof of Theorem \ref{theorem:simple matrices} depends on the field $F$ when using Lemma \ref{Lemma:how to make the simple matrices}. By adapting the construction of $\textup{aGL}_\Lambda (P)$ it might be possible to build an even bigger class of simple topological groups.

\begin{defi}
Let $P_1,\ P_2$ be rings such that $P_1\subset P_2$,\ that is,\ $P_1$ is a subring of $P_2$. Given a proset $\Lambda$ and $A\in \textup{aGL}_\Lambda(P_2)$,\ define the singularities of $A$ in relation to $P_1$ as:
$$S_{P_1}(A)=\{(s_1,\ s_2):\ A_{s_1,s_2}\in P_2\backslash P_1\}\subset \Lambda\times \Lambda.$$
We then define the group $\textup{aGL}_\Lambda(P_2,\ P_1)$ as follows:
$$\textup{aGL}_\Lambda(P_2,\ P_1)=\{A\in \textup{aGL}_\Lambda(P_2):\ S_{P_1}(A) \text{ is finite}\}.$$
\end{defi}

In a similar way to what we had for the case $\textup{aGL}_\Lambda(P)$ it might be possible to prove the following:

\begin{conjecture}
Let $P_1,\ P_2$ be rings such that $P_1$ is a subring of $P_2$. Then $\textup{aGL}_\Lambda(P_2,\ P_1)=\varinjlim_{S\subset \Lambda \text{finite}}(\textup{aGL}_{\Lambda}(P_1)+\textup{GL}_{\overline{S}}(P_2))$,\ where $\overline{S}$ is the proset with elements in $S$ and order given by all elements being equivalent. 
\end{conjecture}

\begin{conjecture}
Let $F$ be a topological field,\ $R$ a closed subring of $F$ and $\Lambda$ an infinite, locally finite proset. Then $Z(\textup{aGL}_\Lambda(F,\ P))=Z(\textup{aGL}_\Lambda(P))$ and it is the unique largest closed subgroup of $\textup{aGL}_\Lambda(F,\ P)$. In particular,\ $\textup{aPGL}_\Lambda(F,\ P):=\textup{aGL}_\Lambda(F,\ P)/Z(\textup{aGL}_\Lambda(P))$ is topologically simple. 
\end{conjecture}

Another construction can be made by allowing some coordinates to be from different rings. For example,\ let $\{P_n\}_{n\in\mathbb{N}}$ be a collection of rings such that $P_{n+1}$ is an $P_k$-algebra,\ for all $k\leqslant n+1$. Let $s_1\preceq s_2\in \Lambda$. Define the length of the interval $[s_1,\ s_2]$ as
$$l([s_1,\ s_2])=\left\{\begin{array}{ll}
   0  & \mbox{if }s_1\sim s_2 \\
   n+1  & \mbox{if there are }t_0=s_1\precnsim t_1\precnsim t_2\precnsim \ldots\precnsim t_{n}=s_2 \mbox{ such that } t_i\preceq t \preceq t_{i+1} \\
&   \text{then either } t_i\sim t \text{ or }t\sim t_{i+1}. 
\end{array}\right.$$
We then can define $\textup{M}_{\Lambda}(\{P_n\}_{n\in\mathbb{N}})$ the set of matrices such that if $l([s_1,\ s_2])=n$ then $A_{s_1,s_2}\in P_n$. Multiplication and addition are defined coordinatewise as for the matrices $\textup{M}_{\Lambda}(P)$.\\
\indent The finitary incidence algebras, as defined in \cite{Matrices2010}, might give rise to other interesting examples of topological groups. An extension of the incidence functor to the whole category $\mathbf{prosets}$, not just the locally finite ones, might be possible as well.

==> Sections/draft.tex <==

We want to describe $\Lambda_{j_0,k_0}$ and maps $p_1,p_2$ such that the diagram is a pushout diagram. As $\Lambda_{f,g}$ is written as a coproduct we can define $p_1$ and $p_2$ on each one of its components, and then it will be uniquely defined for the entire set.\\
\indent For $j\neq j_0$, define $p_1|_{\Lambda_j}:\Lambda_j\rightarrow \Lambda_{f,g}$ as the convex embedding that maps such that $p_1|_{\Lambda_j}(\Lambda_j)=\Lambda_j$. In a similar way, define $p_2|_{\Lambda_k}:\Lambda_k\rightarrow \Lambda_{f,g}$ for all $k\neq k_0$.\\
\indent It remains to define $\Lambda_{j_0,k_0}$ and $p_1,p_2$ for such component. For that we have the following cases
\begin{enumerate}[label=\roman*]
    \item Both $f,g$ are convex embeddings.
    \item Both $f,g$ are constant functions.
    \item Either $f$ or $g$ is a convex embedding.
\end{enumerate}
Notice that the case $\Lambda=1$ is included in i and ii. For cases i and ii, define the set of elements of $\Lambda_{j_0,k_0}$ as the quotient set $(\Lambda_{j_0}\sqcup \Lambda_{k_0})/\sim$ with equivalence relation given by for every $t\in \Lambda$, $f(t)\sim g(t)$ in $\Lambda_{j_0}\sqcup \Lambda_{k_0}$. Define the order in such set as $s_1\preceq s_2$ in $\Lambda_{j_0,k_0}$ if one of the following is true:
\begin{itemize}
    \item $s_1\preceq s_2$ in $\Lambda_1$,
    \item $s_1\preceq s_2$ in $\Lambda_2$,
    \item $s_1\preceq f(t)$ in $\Lambda_1$ and $g(t)\preceq s_2$ in $\Lambda_2$,
    \item $s_1\preceq g(t)$ in $\Lambda_2$ and $f(t)\preceq s_1$ in $\Lambda_1$. 
\end{itemize}
In an intuitive sense, we are making the disjoint union of $\Lambda_1$ and $\Lambda_2$, gluing the image of $f$ and $g$ and preserving the remaining proset structure. This order is given so that there exists convex embeddings $i_{j_0}$, $i_{k_0}$ from $\Lambda_{j_0}$ and $\Lambda_{k_0}$ into $\Lambda_{j_0,k_0}$ given by the coproduct. Define then $p_1|_{\Lambda_{j_0}}=\pi\circ i_{j_0}$, where the maps $i_{j_0}$ and $\pi$ are the maps $i_{j_0}:\Lambda_{j_0}\rightarrow \Lambda_{j_0}\sqcup \Lambda_{k_0}$, $\pi:\Lambda_{j_0}\sqcup \Lambda_{k_0}\rightarrow \Lambda_{j_0,k_0}$. By the definition of $\Lambda_{j_0,k_0}$, this map is a convex embedding. In a similar way, define $p_2|_{\Lambda_{k_0}}=\pi\circ i_{k_0}$.\\
\indent For the case iii, assume $f$ is a convex embedding and $g$ is constant define $\Lambda_{j_0,k_0}=\Lambda_{k_0}$, $p_2|_{\Lambda_{k_0}}$ the identity map on $\Lambda_{k_0}$, $p_1|_{\Lambda_{j_0}}=\{s\}$, where $s\in \Lambda_{k_0}$ is such that $g(\Lambda)=\{s\}$. We do a similar construction for the case $f$ is constant and $g$ is a convex embedding.\\
\indent Now it remains to prove that such $\Lambda_{f,g}$, $p_1$, $p_2$ form a pushout diagram. By definition, $p_1\circ f=p_2\circ g$. Assume now $f':\Lambda_1\rightarrow \Lambda'$, $g':\Lambda_2\rightarrow \Lambda'$ are such that $f'\circ f=g'\circ g$. We need to show that there exists a unique $p':\Lambda_{f,g}\rightarrow \Lambda'$ that makes the entire diagram commute. For that we define $p'$ in the components of $\Lambda_{f,g}$ and, using the coproduct property, build the desired map.\\
\indent For each $k\in K\backslash\{k_0\}$ define $p'|_{\Lambda_k}=f'|_{\Lambda_k}$. Similarly, for each $j\in J\backslash \{j_0\}$ define $p'|_{\Lambda_j}=f'|_{\Lambda_j}$. We need now to define $p'|_{\Lambda_{j_0,k_0}}$. As $f'\circ f=g'\circ g$, then $f'(\Lambda_{j_0})$ is in the same component as $g'(\Lambda_{k_0})$, and $f'\circ f(\Lambda)$ is contained in their intersection. If $f'$ is constant, let $p'|_{\Lambda_{j_0,k_0}}=g'$ and if $g'$ is constant, let $p'|_{\Lambda_{j_0,k_0}}=f'$. If both $f'$ and $g'$ are convex embeddings, define 
$$p'|_{\Lambda_{j_0,k_0}}(t)=\left\{\begin{array}{ll}
    f'(t) & \text{if }t\in\pi\circ i_{j_0}(\Lambda_{j_0})  \\
    g'(t) & \text{if }t\in\pi\circ i_{k_0}(\Lambda_{k_0}).
\end{array}\right.$$
\noindent As $f'$ and $g'$ are convex embeddings, so is $p'$. It is also the unique function making the whole diagram commute.
